Deploying Near-Optimal Delay-Constrained Paths with Segment Routing in Massive-Scale Networks

With a growing demand for quasi-instantaneous communication services such as real-time video streaming, cloud gaming, and industry 4.0 applications, multi-constraint Traffic Engineering (TE) becomes increasingly important. While legacy TE management planes have proven laborious to deploy, Segment Routing (SR) drastically eases the deployment of TE paths and is thus increasingly adopted by Internet Service Providers (ISP). There is a clear need in computing and deploying Delay-Constrained Least-Cost paths (DCLC) with SR for real-time interactive services. However, most current DCLC solutions are not tailored for SR. They also often lack efficiency or guarantees. Similarly to approximation schemes, we argue that the challenge is to design an algorithm providing both performances and guarantees. However, conversely to most of these schemes, we also consider operational constraints to provide a practical, high-performance implementation. We leverage the inherent limitations of delay measurements and account for the operational constraint added by SR to design a new algorithm, best2cop, providing guarantees and performance in all cases. Best2cop outperforms a state-of-the-art algorithm on both random and real networks of up to 1000 nodes. Relying on commodity hardware with a single thread, our algorithm retrieves all non-superfluous 3-dimensional routes in only 250ms and 100ms respectively. This execution time is further reduced using multiple threads, as the design of best2cop enables a speedup almost linear in the number of cores. Finally, we extend best2cop to deal with massive scale ISP by leveraging the multi-area partitioning of these deployments. Thanks to our new topology generator specifically designed to model the realistic patterns of such massive IP networks, we show that best2cop solves DCLC-SR in approximately 1 second even for ISP having more than 100000 routers.

==> clean_latex/sections/background.tex <==

\section{Back to the Future: DCLC vs SR}\label{sec:background}

\subsection{Segment Routing Background and Practical Usages}
% \paragraph{Segment Routing in a Nutshell}
% What's SR ? Need for SR Graph

\red{Segment Routing implements source routing by prepending packets with a stack of up to MSD \textit{segments}. In a nutshell, segments are checkpoints the packet has to go through.
There are two main types of segments}:
\begin{itemize}
    \item \textbf{Node segments.} A node segment $v$ indicates that the packet should (first) be forwarded to $v$ with ECMP (instead of its final IP destination). Flows are then load-balanced among the best IGP next hops for destination $v$.
    \item \textbf{Adjacency segments.} Adjacency segments indicate that the packet should be forwarded through a specific interface and its link.
\end{itemize}

\red{Once computed, the stack of segments encoding the desired path is added to the packet. Routers forward packets according to the topmost segment, which is removed from the stack when the packet reaches the associated intermediate destination.}

% and may either specify a node (such segments are called \textit{node segments}), or an interface and its link (\textit{adjacency segments}).

Adjacency segments may be globally advertised, and thus be used the same way as node segments, or they may only have a local scope and, as such, can only be interpreted by the router possessing said interface. In this case, the packet should first be guided to the corresponding router, by prepending the associated node segment. \red{In the following, as a worst operational case, we consider the latter scenario, as it
always requires the highest number of segments.}

% Indeed, the resulting number of segments can be seen as an upper bound, as node segments preceding adjacency ones could be removed depending on the control-plane in use (\ie if adjacency segments are globally advertised).

Segment Routing attracted a lot of interest from the research community. A table
referencing most SR-related work can be found in Ventre et al.~\cite{ventre_segment_2020}. While some SR-TE works are related to tactical TE problems (like minimizing the maximum link utilization) taking indirectly into account some delay concerns~\cite{swarm, 10.1007/978-3-319-23219-5_41}, most of the works related to SR do not focus on DCLC, but rather bandwidth optimization ~\cite{7218434,Gay2017ExpectTU, Loops}, network resiliency \cite{8406885, 7524551}, monitoring~\cite{SRv6PM, 7524410}, limiting energy consumption ~\cite{7057272} or path encoding (the translation of path to segment lists)~\cite{guedrez2016label,7417097}. Aubry~\cite{AubryPhd}
proposes a way to compute paths requiring less than MSD segments while optimizing
an additive metric in polynomial time. The number of segments required is then evaluated. This work,
however, considers only a single metric in addition to the operational constraints.
The problem we tackle
(\ie DCLC paths for Segment Routing) deals with two metrics (in addition to the operational constraints). This additional dimension drastically changes the problem,
which then becomes NP-Hard.
Some works use a construct similar to ours (presented in details in Sec.~\ref{sec:sr-graph}) in order to prevent the need to perform conversions from network paths to segment lists, \cite{Lazzeri2015EfficientLE} in particular. However, the authors of \cite{Lazzeri2015EfficientLE} do not pretend to solve DCLC and, as such, do not tune the structure the same way
(\ie they do not remove dominated segments, as explained later on), and simply use their construct to sort paths lexicographically.

%These segments may be globally advertised, allowing routers to load balance the packets towards the specified (distant) interface directly as if it were a node, or they only have a local scope, and routers first need to forward packets to the invertex of the specified link, requiring so an additional node segment. Once arrived at this node, the adjacency segment can be interpreted as it describes a local interface.
As aforementioned, while operators seem to mainly deploy SR to perform fine-grained TE, to the best of our knowledge, no DCLC variant exists for specifically tackling SR characteristics and constraints (except for our contribution).
Using segments to steer particular flows allows however to deviate some TE traffic from the best IGP paths
in order to achieve, for example, a lower latency (and by extension solve DCLC). A realistic example is shown on Fig.~\ref{fig:DCLCGeant} where the node segment \textit{Vienna}, as well as considering Vienna as the destination itself, would result in the packets following the best IGP path from Frankfurt to Vienna, i.e., the green dashed path.
To use the direct link instead (in plain pink) and so minimize the delay between the two nodes of this example, the associated adjacency segment would have to be used as it enforces a single link path having a smaller delay than the best IGP one (including here two intermediary routers).
Finally, the yellow path, offering a non dominated compromise between both metrics (and being the best option if considering a delay constraint of 8ms), requires the use of the node segment \textit{Budapest} to force the traffic to deviate from its best IGP path in green.
Before converting the paths to segment lists (and actually deploy them with SR), such non-dominated paths need first to be explored.
Computing these paths while ensuring that the number of segments necessary to encode them remains under MSD is at least as difficult as solving the standard DCLC problem since an additional constraint now applies.


% we would have DCLC-SR$(\mathit{Frankfurt}, 3, 8) \supset \mathit{Frankfurt}-\mathit{Budapest}-\mathit{Vienna}$ (the yellow path made of one segment towards Budapest, is the best option for the specific Vienna destination considering an arbitrary delay constraint of 8ms (the best IGP path towards Vienna being the green one, the DCLC path requires at least one segment)



% TODO: PUT THIS ELSEWHERE MAYBE
% To natively encompass SR and its related constraint, MSD, we propose a structure from which the IGP costs, delays, as well as the type and number of segments encoding a given path can be directly manipulated in order to avoid any superfluous operations (e.g. exploring or converting paths not encodable with less than MSD segments).
% This construct, called the multi-metric SR-graph, is detailed in section \ref{sec:srgraph}.


%direct and natural properties.


\subsection{DCLC (Delay-Constrained, Least-Cost), a Well-known Difficult Problem having many Solutions?}

%\cite{survey98, survey02, survey2010, survey2018,Karaboga})
DCLC belongs to the set of NP-Hard problems (as well as most related multi-constrained path problems).
Intuitively, solely extending the least-cost path is not sufficient, as the latter may exceed the delay constraint.
Thus, paths with greater cost but lower delays must be memorized and extended as well.
These \textit{non-dominated paths} form the \textit{Pareto front} of the solution, whose size may grow exponentially with respect to the size of the graph.
However, DCLC in particular, and related variants and extensions in general, does possess several interesting applications such as mapping specific flows to their appropriate paths (in terms of interactive quality).
Thus, these problems have been extensively studied in the past decades.
Many solutions have been proposed so far, as summarized in these surveys~\cite{survey02, survey2010, survey2018}: they range from to heuristics and approximations to exact algorithms, or even genetic approaches.\\


%Because of this, algorithms able to solve DCLC exactly exhibits an exponential
%worst-case complexity.

%NOTE :Left out DEB -- Dual extended Bellman Ford. DEB uses a BFord-like algorithm to compute
% ALL path of k hops in order to increase its chance of finding a feasible path

% OLD VERSION
% Because DCLC is NP-Hard, several heuristics have been designed. The latter offer no guarantees but possess a low time complexity. Some heuristics solely rely on the knowledge of the least cost (LC) and least delay (LD) paths. \cite{Fallback} returns either the LC or LD path if one is feasible (\ie respect the constraints). DCBF~\cite{DCBFKLARAC} computes the shortest paths through a Bellman-Ford procedure, but only relaxes paths that seem feasible.
% Most heuristics try to explore the delay and cost dimension simultaneously. \cite{DCUR, DCR} allow each node to select either the LC or LD path to the next node. These solutions have been extended in \cite{SFDCLC} and \cite{SMM}.
% Other heuristics combine the cost and the delay into a single linear aggregated metric to be able to use a standard shortest path algorithm~\cite{Jaffe}. LARAC-based methods~\cite{Aneja_Nair_1978}, in particular, perform several Dijkstra runs with different aggregated costs to find the best way to aggregate both metrics.
% Methods relying on linear costs can however only find paths on the convex hull of the Pareto front and may thus miss paths. To mitigate this effect, the latter may use a $k$-shortest paths algorithm
% to increase the chance of discovering additional non-dominated paths~\cite{DCBFKLARAC, larac}.
% Nevertheless, linearly aggregating metrics necessarily leads to loss of relevant information regarding the quality and feasibility of the explored paths~\cite{536364}.

% Thus, some algorithms explore the solution space in a non-linear fashion, allowing them to better scan the feasible space. However, in this case, the optimality of subpaths does not hold. Solutions should thus maintain and extend a potentially exponential member of (non-dominated) paths at each node. Both TAMCRA~\cite{TAMCRA} and LPH~\cite{EBFA01} maintain and extend up to $k$ non-dominated paths per node, discovered either through a PQ with a non-linear aggregated metric or a Bellman-Ford approach respectively.
% HMCOP~\cite{Korkmaz_Krunz_2001} first runs a standard Dijkstra algorithm to gain some knowledge regarding the feasibility of the paths. This knowledge is used in the next execution which explores the paths through a PQ and a non-linear cost.
% Finally, ~\cite{Feng_Makki_Pissinou_Douligeris_2002, Guo_Matta_1999} rely on MCP algorithms (which find feasible paths with no optimization objective), using a conservative cost constraint refined iteratively.

\textbf{Heuristics.} Because DCLC is NP-Hard, several polynomial-time heuristics have been designed to limit the worst-case computing time, but at the detriment of any guarantees.
For example, \cite{Fallback} only returns the least-cost or least-delay path
if one is feasible (\ie respect the constraints).
More advanced proposals try to explore the delay and cost space simultaneously, by either combining in a distributed manner the least-cost and least-delay subpaths~\cite{DCUR, DCR, SFDCLC} or by aggregating both metrics into one in a
more or less intricate manner.

Aggregating metrics in a linear fashion~\cite{Jaffe, Aneja_Nair_1978}
preserves the \textit{subpaths optimality principle} (isotonicity of best single-metric paths) and therefore allows to use standard shortest paths
algorithms. However, it leads to a loss of relevant information regarding the quality
and feasibility of the computed paths~\cite{536364}, in particular if the hull of the Pareto Front is not convex. Some methods try to mitigate this effect by using a $k$-shortest path approach to possibly find more feasible paths~\cite{DCBFKLARAC, larac}, but such an extension may result in a large increase of execution time and may not provide more guarantees.
% JRO: Left out \cite{SMM}, which is like DCUR and DCR but allows a node to choose from more paths then
% just the LC or LD one. Don't really know where it would fit.
Other heuristics rely on non-linear metric aggregation.
While it seems to prevent loss of relevant information, at first glance, such algorithms expose themselves to maintain all non-dominated paths (towards all nodes) as the isotonicity does not hold anymore (while it holds with linear metrics). Since the Pareto Front may be exponential with respect to the size of the graph, those algorithms either simply impose a hard limit on the number of paths that can be maintained (\eg TAMCRA~\cite{TAMCRA} and LPH~\cite{EBFA01}), or specifically chose the ones to maintain through previously acquired knowledge (HMCOP~\cite{Korkmaz_Krunz_2001}).
Finally, other works like~\cite{Feng_Makki_Pissinou_Douligeris_2002, Guo_Matta_1999} rely on heuristics designed to solve a variant of DCLC, the MCP problem (Multi-Constrained Paths, the underlying NP-Complete decision version of DCLC -- with no optimization objective). It mainly consists of sequential MCP runs using a conservative cost constraint iteratively refined.
% Their optimality and execution time drastically rely on the underlying MCP algorithm.

Relying on heuristics is tempting, but their lack of guarantees can prevent to enforce strict SLAs even when a suitable path actually exists. %an important feature when deploying fine-grained TE.
One can argue it is particularly unfortunate, as DCLC is only \textit{weakly} NP-hard: it can be solved exactly in pseudo-polynomial time, \ie polynomial in the numerical value of the input~\cite{gareycomputers}.
Said otherwise, DCLC is polynomial in the smallest largest weight of the two metrics once translated to integers.
Consequently, it is possible to design FPTAS\footnote{Fully Polynomial Time Approximation Scheme.} solving DCLC while offering strong guarantees~\cite{Papadimitriou_Yannakakis_2000}.\\

%
\textbf{Approximations.}
\red{Numerous FPTAS have been proposed to solve DCLC and related constrained shortest path problems. All the following algorithms fall into this category.}
The common principle behind these schemes is to reduce the precision (and/or magnitude) of the considered metrics.
This can be performed either directly, by \textit{scaling and rounding} the weights of each link, or indirectly,
by dividing the solution space into intervals and only maintaining paths belonging to different intervals (\textit{Interval partitioning})~\cite{Sahni_1977}.
Scaling methods usually consider either a high-level dynamic programming scheme or a low-level practical Dijkstra/Bellman-Ford core with pseudo-polynomial complexity, and round the link costs to turn their algorithms into an FPTAS (see for example Hassin~\cite{Hassin_1992}, Ergun et al.~\cite{Ergun_Sinha_Zhang_2002} or Lorenz and Raz~\cite{Lorenz_Raz_2001} methods).
Goel et al.~\cite{goel}, in particular, chose to round the delay instead of the cost and can consider multiple destinations (as our own algorithm).
%The path found may thus violate the delay constraint by a factor $(1+\epsilon)$, but will possess the lowest cost. Their method is also able to compute DCLC paths for multiple destination, a fairly rare feature in such algorithms.
% Note perso: left out \cite{Warburton_1987}

Most interval partitioning solutions explore the graph through a Bellman-Ford approach.
The costs of the paths are mapped to intervals, and only the path with
the lowest delay within a given interval is kept. The size of the intervals
thus introduces a bounded error factor~\cite{Hassin_1992, Tsaggouris_Zaroliagis_2009}.
In particular, HIPH~\cite{HIPH} offers a dynamic approach between an approximation and exact scheme. It proposes to maintain up to $x$ non-dominated paths for each node and stores eventual additional paths using an interval partitioning strategy. This allows the algorithm to be exact on simple instances (resulting in a limited Pareto front, \ie polynomial in the number of nodes, in particular when it is bounded by $x$) and offer strong guarantees on more complex ones. This versatility is an interesting feature, as most real-life cases are expected to be simple instances with a bounded Pareto front size, in particular because one of the metrics may be coarse by nature. % (while the reciprocal is not granted).
For these reasons, not only approximation schemes can offer practical solutions (with a bounded margin error) but also exact algorithms (with controlled performance), as they may be viable in terms of computing time for simple real-life IP networking instances.\\
%and have thus also been studied extensively.
% NOTE JRO : I didn't say that they have the best delay per cost interval but may
% maintain dominated paths (non dominancy check between intervals)

%Exact algorithms solving DCLC usually rely on the same optimality principle as standard shortest path algorithms (parts of shortest paths are shortest paths themselves), but adapted to multi-metric problems
%(parts of a non-dominated path are non-dominated paths themselves). Thus, all non-dominated paths to a given node are extended.


\textbf{Exact methods.} Numerous exact methods have indeed also been studied extensively to solve DCLC.
Some methods simply use a $k$-shortest path approach to list all paths within the Pareto front~\cite{Namorado_Climaco_Queiros_Vieira_Martins_1982, Paixao_Santos_2008}.
On the other hand, Constrained Bellman-Ford~\cite{CBF94} (ironically, also called Constrained Dijkstra as it uses a priority queue -- denoted PQ in the following) explores paths by increasing delays and lists all non-dominated paths towards each node.
%Of course, since several non-dominated paths exists to a given node, the paths (and their costs) themselves are kept within the PQ (instead
%of the corresponding node in standard shortest path algorithms).
Several algorithms use the same principle but order the paths differently within the queue, relying either on a lexicographical ordering, ordered aggregated sums, or a simple FIFO/LIFO ordering~\cite{Martins_1984, Martins_Santos_1999,Brumbaugh-Smith_Shier_1989}. Most notably, A* Prune~\cite{Liu_Ramakrishnan_2001} is a multi-metric adaptation\footnote{This adaptation is exact, \ie not a heuristic, as the estimated cost underestimates the actual distance towards the destination.} of A* relying on a PQ where paths known to be unfeasible are pruned. % thanks to pre-computations and is thus exact when the computed look-ahead is conservative enough.
%However, the latter are not trivial to generalize to deal with more than two metrics.
Two-phase methods~\cite{Raith_Ehrgott_2009} first find paths
lying on the convex hull of the Pareto front through multiple Dijkstra runs,
before finding the remaining non-dominated path through implicit enumerations.
%The knowledge gained in this first phase then allows to find the resulting
%non-dominated paths through a branch-and-bound algorithm or a similar method.

Finally, \samcra~\cite{SAMCRA} is a popular and well-known multi-constrained path algorithm.
Similarly to other Dijkstra-based algorithms, \samcra relies on a PQ
to explore the graph but instead of the traditional lexicographical ordering, it relies on non-linear cost aggregation.
Among feasible paths (others are natively ignored) it first considers the one that minimizes its maximum distance to the multiple constraints. Such a path ranking to deal with the PQ is supposed to increase its performance with respect to other PQ organizations.


\begin{table*}[!ht]
    \centering
    \caption{Qualitative summary of a representative subset of DCLC-compatible algorithms showcasing their practicality, exactitude, and performance. In the \textit{Practical Features} column, the green check-mark indicates whether the algorithm supports the corresponding feature (while the red cross denotes the opposite). In the \textit{Exactitude vs Performance} column, the two subcolumns associated which each three scenarios show how the latter impact $(i)$ the exactitude (exact, strong guarantees, no guarantees) and $(ii)$ the performance of the algorithm (polynomial time or not). While the orange tilde denotes strong guarantees in terms of exactitude, green check-marks (and red crosses respectively) either indicate exact results (no guarantees resp.) or polynomial-time execution (exponential at worst resp.) for performance. For both subcolumns \textit{Bounded Pareto Front} and \textit{Coarse Metric}, we consider the case where their spreading is polynomial with respect to the number of vertices in the input graph (and as such predictable in the design/calibration of the algorithm).
    }
    \label{tab:relatedtable}
    \begin{tabular}{cccccccccc}
    \toprule
              Algorithms   & \multicolumn{3}{c}{Practical Features} & \multicolumn{6}{c}{Exactitude vs Performance}   \\
              \cmidrule(r){2-4}\cmidrule(l){5-10}
                  & Multi-Dest & SR   & Multi-thread & \multicolumn{2}{c}{Bounded} & \multicolumn{2}{c}{Coarse}  & \multicolumn{2}{c}{All} \\
                  & Single Run & Ready & Ready & \multicolumn{2}{c}{Pareto Front} & \multicolumn{2}{c}{Metric} & \multicolumn{2}{c}{Cases}  \\\midrule
    LARAC~\cite{larac} &  \darkredcross     & \darkredcross     & \darkredcross               & \darkredcross & \darkgreencheck & \darkredcross & \darkgreencheck & \darkredcross      & \darkgreencheck     \\
    LPH~\cite{EBFA01}   &  \darkgreencheck     & \darkredcross     & \darkredcross               & \darkgreencheck & \darkgreencheck & \orangetilde & \darkgreencheck & \darkredcross      & \darkgreencheck     \\
    HMCOP~\cite{Korkmaz_Krunz_2001}   &  \darkredcross     & \darkredcross     & \darkredcross  & \darkredcross & \darkgreencheck & \darkredcross & \darkgreencheck & \darkredcross      & \darkgreencheck     \\ \midrule
    HIPH ~\cite{HIPH}  &  \darkgreencheck    & \darkredcross     & \darkredcross               & \darkgreencheck & \darkgreencheck & \darkgreencheck      & \darkgreencheck & \orangetilde      & \darkgreencheck     \\
    Hassin~\cite{Hassin_1992} &  \darkredcross    & \darkredcross     & \darkredcross               & \orangetilde      & \darkgreencheck & \darkgreencheck     & \darkgreencheck & \orangetilde           & \darkgreencheck     \\
    Tsaggouris et al.~\cite{Tsaggouris_Zaroliagis_2009} & \darkgreencheck & \darkredcross & \darkredcross & \orangetilde & \darkgreencheck & \darkgreencheck & \darkgreencheck & \orangetilde & \darkgreencheck \\\midrule
    Raith et al.~\cite{Raith_Ehrgott_2009}  & \darkredcross & \darkredcross     & \darkredcross               & \darkgreencheck & \darkgreencheck      & \darkgreencheck & \darkgreencheck     & \darkgreencheck      & \darkredcross     \\
    A* Prune.~\cite{Liu_Ramakrishnan_2001}  & \darkredcross & \darkredcross     & \darkredcross               & \darkgreencheck & \darkgreencheck      & \darkgreencheck & \darkgreencheck     & \darkgreencheck      & \darkredcross     \\
    SAMCRA~\cite{SAMCRA} &  \darkgreencheck     & \darkredcross     & \darkredcross               & \darkgreencheck & \darkgreencheck      & \darkgreencheck & \darkgreencheck      & \darkgreencheck      & \darkredcross     \\ \midrule\midrule
    BEST2COP  & \darkgreencheck  & \darkgreencheck     & \darkgreencheck               & \darkgreencheck & \darkgreencheck  & \darkgreencheck & \darkgreencheck  & \orangetilde    & \darkgreencheck    \\ \bottomrule
    \end{tabular}
    \end{table*}


% This non-linear cost can
%be adapted to better fit some particular constrained path problems.
% SAMCRA has been extended to
%support additional features such as look-aheads.

As we have seen so far, while many solutions exist, most possess certain drawbacks or lack certain features to reconcile both the practice and the theory.
Heuristics do not always allow to retrieve the existing paths enforcing strict SLAs, while exact solutions
are not able to guarantee a reasonable maximum running time when difficult instances arise, although both features are essential for real-life deployment.
On the other hand, FPTAS can provide both strong guarantees and a polynomial execution time.
However, they are often found in the field of operational research where, at best, possible networking applications and assumptions are discussed, but are not investigated.
Because of this, the deployment of the computed paths, with SR and its MSD in particular, is not taken into consideration. It is worth to note that the number of segments
is not a standard metric as it is not simply a weight assigned to each edge in the original graph (that is, without a specific construct, it requires to be computed on the fly for each visited path). Considering the latter can have a drastic impact on the performance of the algorithms not designed with this additional metric in mind.
In addition, not all the algorithms presented here and in Table~\ref{tab:relatedtable} are single-source multiple-destinations. Finally, none of these algorithms
evoke the possibility to leverage multi-threaded architectures, an increasingly important feature as such computations now tend to be performed by dedicated Path Computation Elements or even in the cloud.


% JRO: le terme practically exact est probablement très/trop foireux
Our contribution, \bestcop, aims to close this gap by mixing the best existing features (such as providing both a limited execution time and strong guarantees in terms of precision in any cases) and adapt them for a practical modern usage in IP networks deploying SR.
Table~\ref{tab:relatedtable} summarizes some key features of a representative subset
of the related work. Similarly to FPTAS, \bestcop rounds one of the metrics of the graph. However, conversely to most algorithms,
% except ~\cite{Goel}
\bestcop does not sacrifice accuracy of the cost metric, but of the measured delay. Because of the native inaccuracy of delay measurements (and the
arbitrary nature of its constraint), this does not prevent \bestcop from being technically exact in most practical cases.
% when the aforementioned accuracy is coarse
%enough and/or the delay constraint strict enough
% (\eg around the millisecond for a constraint of 100ms, or around
%the microsecond fot a constraint of 10ms).
In addition (and akin to ~\cite{HIPH}), \bestcop can easily be tuned to remain exact on all simple instances with a bounded Pareto front regardless of the accuracy of the metrics. Thus, \bestcop can claim to return exact solutions in most scenarios and, at worst, ensure strict guarantees in others (for theoretical exponential instances). In all cases, \bestcop possesses a pseudo-polynomial worst-case time complexity. \bestcop
was designed while keeping the path deployment aspect of the problem in mind. A single run allows to find all DCLC paths (and many variants as we will see later) to all destinations. The MSD constraint related to SR is taken into account
natively. As a result, paths requiring more than MSD segments are excluded from the exploration space. The outer loop of \bestcop can be easily parallelized, leading to a non-negligible reduction in the execution time.
In Sec.~\ref{sec:evaluation}, relying on a performance comparison between \bestcop and \samcra, we will show that \bestcop does not even need to rely on multi-threading to provide lower computing times than \samcra while returning the exact same solutions (even though we make \samcra benefit from advantageous methods explained thoroughly in the remainder of this paper).
This result is particularly interesting as it remains true even for simple IP network instances. This comparison also enables to evaluate Dijkstra-oriented solutions (\samcra) with respect to Bellman-Ford-oriented ones (\bestcop).

%  (and also letting \samcra benefiting from our advantageous SR construct\footnote{We make \samcra benefit from both discretized delays and the multi-metric SR graph, as explained more thoroughly in the remainder of this paper. This comparison also enables to evaluate Dijkstra-oriented solutions (\samcra) with respect to Bellman-Ford-oriented ones (\bestcop).}

%that do not require to manage a PQ as the path exploration is natively and iteratively guided by the number of hops/segments in the paths.}).
Last but not least, \bestcop has been adapted for multi-area networks and leverages the structures of the latter, allowing it to solve DCLC on very large ($\approx$ \num{105000} nodes) domains in one second. To the best of our knowledge, such large-scale experiments and results have neither been conducted nor achieved within SR domains~\footnote{Some elementary algorithms (such as Multi-constrained Dijkstra) and more intricate solutions exhibit impressive computing times on even more massive road networks~\cite{Hanusse_Ilcinkas_Lentz_2020}. However, such networks are less dense than IP ones (and with metrics that are also even more correlated).}.

















%The red crosses and green checkmarks in the \textit{Practicality} column shows if the algorithm can support
%    natively the associated feature, \ie the ability to solve DCLC for all destinations in a single run, the support of Segment Routing,
%    and the support of multi-threading. Note that some algorithms may be parallelized, but no mention of parallelization were
%    present in the associated paper. The columns \textit{Small Pareto Front}, \textit{Coarse Metric} and \textit{All Cases} are
%    divided into two subcolumns, showing (i) if the corresponding algorithm is exact in this scenario and (ii) if the algorithm
%    showcases good performances in this scenario. A green checkmark in the first subcolumn means that the algorithm is
%    exact in the corresponding scenario, while an orange tilde means this algorithm is not exact but has strong guarantees. Finally,
%    a red cross means the algorithm has no guarantess. Similarly, a green checkmark in the second subcolumn means
%    that the algorithm has good performance in the given scenario, while a red checkmark shows that the algorithms
%    may exhibit long runtime. Finally, an orange tilde means that altough the scenario may have an impact on the usual
%    performance of the algorithm, but the latter are still dependant on the instance of the problem.
%
% Small Pfront for exact method => check mark for performance ?




    % In this paper, we compare ourselves to \samcra, being more recent and popular than most of the algorithms presented here and able to compute constrained paths for all destinations. This choice also enables to compare Dijkstra-oriented solutions to Bellman-Ford-oriented ones. We make \samcra benefit from both
    % discretized delays and our construct used to encompass SR, as explained more thoroughly in the remainder of this paper.

% Note JRO: transition de toute façon un peu brutale, donc j'ai décidé de virer le paragraphe en commentaire ci dessous, mais je le laisse en comment au cas où

%The requirement of such construct and the added complexity brought
%by SR (and the MSD constraint) bring forth an essential preliminary question.
%Although SR is the new standard for TE paths deployement, the fact that only paths encodable by MSD segments at most can be deployed may seem like an issue.
%Can SR be used for fine-grained TE such as the deployment of DCLC paths, or is the MSD constraint too strict?


\subsection{SR is Relevant for DCLC: MSD is not a Limit}~\label{ssec:nbseg}

Given the MSD constraint, one may question the choice of SR for deploying DCLC paths in practice.
Indeed, in some cases, in particular if the metrics are not aligned\footnote{The delay and the IGP costs in particular. Since node segments represent best IGP paths, the IGP cost and the number of segments will most likely be aligned by design}, constrained paths
may required more than MSD detours to satisfy a
stringent latency constraint.
% since SR builds its set of segments based on the IGP metric, the number of segments and the IGP are aligned by design}, some DCLC paths could require more than MSD segments.
% Constrained paths could require more than MSD segments if numerous detours become necessary to satisfy tight delay constraints.
% Indeed, when metrics are not aligned,
% % ($M_1$ and $M_2$ in particular as $M_0$ and $M_2$ are aligned by design
% % (, as the IGP and the number of segments are aligned by design\footnote{Low IGP distances are, by construction, achievable with few segments as shortest distances require only one segment since SR builds its set of segments based on the IGP metric by default.})
% % , each link of the resulting DCLC path may require to be individually forced with its counterpart adjacency segment.
% % Thus, in theory,
% some constrained paths may lead to a segment list exceeding MSD.


\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{all-dclc-paths.pdf}
    \caption{Required number of segments for all DCLC solutions, in a network of \num{45000} nodes generated by YARGG, with delay constraints of up to \num{100}ms.}
    \label{fig:nbseg}
\end{figure}



% Removed "flex algo"
While it has been shown that few segments are required for most current SR usages (e.g. for TI-LFA \footnote{Topology Independent Loop Free Alternate} or when considering only one metric)~\cite{TheseClarenceFils,AubryPhd}, to the best of our knowledge, there is no similar study for our specific use-case, i.e. massive scale networks with two valuation functions (delay and IGP cost).
This is probably one of the most exciting challenge for SR as DCLC is a complex application.
However, since such massive-scale computer network topologies are not available publicly, we rely on our own topology generator whose detailed description is available in section \ref{sec:generator}.
% Our aim is to obtain realistic networks and patterns benefiting from both the physical hierarchy and metrics alignement observed in real cases like in Fig.~\ref{fig:DCLCGeant}.
These topologies follow a standard OSPF-like area division.
and both metrics (delay and IGP cost) follow a realistic pattern. For this analysis, we opt for a worst-case graph having $\approx~$\num{45000} nodes and $\approx~$\num{92000} edges scattered in \num{140} areas.


For this analysis, we keep track, for each destination, of all the solutions solving DCLC for all delay constraints up to 100ms, and extract the necessary number of segments.
% \ie, DCLC-SR with $c_0 = MSD = \infty$, and we examine the necessary number of segments.
% for all longest segment paths.
In other words, we show the number of segments required to encode all non-dominated (and thus practically relevant for some given constraint) paths, considering all delay constraints up to 100ms.
The results are shown in Fig.~\ref{fig:nbseg}.
% in which the term \textit{NA} refers to cases where there were no feasible paths towards a given destination.
% It is worth noticing that the looser $c_1$ is, the fewer segments are required (here 5ms represents a rather difficult challenge). Since $M_0$ and $M_2$ are aligned by construction, loose delay constraint allow the shortest IGP paths (requiring very few segments) to be feasible (and become the optimal DCLC solution).


%In the extrem case where $c_1 = \infty$ no segment is needed at all as the best IGP routes are the selected by default by the routers.\QB{en fait je sais pas si c'est worth noticing ici}
% Conversely, since 2COP encompasses other problems (\eg minimizing $M_1$, which does not align with $M_0$), loose $c_1$ constraints allow for more relevant path to become feasible.

% While the MSD limit does not seem to be an issue for most configurations (as most paths do not require more than 10 segments), %, in particular DCLC ones \QB{pas sur de comprendre le "in particular DCLC ones", car la discussion est uniquement sur les solution DCLC justement non?)}),
% it can be a problem for random weighted graphs. The MSD constraint brought by SR does indeed prevent it from reaching some feasible paths on random topologies: for a significant share of source-destination pairs, there exist non-dominated solutions requiring more than 10 segments. This implies that, for such pairs on such graphs, there exist constraints where the optimal solution cannot be deployed using SR.

\red{One can see that most paths require less than 10 segments,
meaning that performant hardware should be able to
deploy most DCLC paths. However, some corner-cases requiring more than 10 segments do exist, probably arising
from stringent delay constraints. In addition, less performant hardware (\eg with MSD $\approx 5$), while able to deploy the majority of DCLC paths, can not deploy \textit{any} DCLC path. Note that several mechanisms exist to bypass this limit. Flexible Algorithms~\cite{I-D.ietf-lsr-flex-algo} allows to compute shortest paths and create segments with other metrics (\eg the delay). Binding segments~\cite{RFC8402} allows to "compress" a segment list in a single segment, which is uncompressed when popped from the list. However, both techniques increases the message exchange, number of states to maintain, and overall complexity. Their usage should thus be limited to a few corner cases.}

\red{Consequently, our analysis exhibits two main points. First, SR is appropriate to deploy TE paths. Indeed, the majority of DCLC paths should be deployable within the MSD constraint, if not all when using performant hardware. Second, since there may however exist DCLC paths requiring more than MSD segments, this limit \text{must} be considered to compute feasible paths correctly. Otherwise, a single non-feasible path dominating feasible ones is enough to lead to an incorrect algorithm. The underlying path computation algorithm must then efficiently consider delay, IGP cost and the number of segments to ensure its correctness.}

% One can see that the MSD limit (if we consider the latter to be $\approx 10$) does not seem to be an issue for most
% configurations, as most paths require less than 10 segments.
% Said differently, we have DCLC-SR = DCLC in most cases for the best performing hardware. However,
% even when considering realistic IGP weights and delay, there exist some corner cases which require more than 10 segments, probably arising from stringent delay constraints.
% These cases probably arise from
% stringent delay constraint (recall that we consider all constraints $\leq 100$), for which adequate paths may require a larger number of segments than usual.

%In any cases, the number of segment has to be considered when computing paths.

% On realistic topologies, the alignment of the metrics greatly reduces this effect: all feasible solutions are reachable with less than 10 segments.
%Thus, while SR may prevent from deploying non dominated solutions for some corner cases, real network
%characteristics seem to reduce the number of required segments drastically.
%The MSD limitation thus mostly concerns random graphs and, even for them, does not hinder the deployment of the most interesting TE paths, the DCLC ones.
%Indeed, while 2COP can be of practical interest, DCLC (included within 2COP) remains the most interesting and popular problem among ISPs.
%For DCLC-SR on realistic weights, one can see that the MSD limit has no effect: DCLC paths required at most TODO segments.

% On realistic topologies, since the three metrics are often aligned (though not perfectly), a few solutions dominate all others on the 3D Pareto front.

% Note that this evaluation shows the \textit{longest} segment list still relevant to the underlying problem.
% Cases for which all feasible distances required more than MSD segments for a given couple source/destination exist for strict constraints, but were extremely rare, only $\approx$0.007\%.
% In other words, for almost \textit{all} cases, although the optimal path could rarely require more than 10 segments, a not optimal but alternative SR-feasible solution existed.

% Note: since we do not used flex algo later, we can remove its explanation
% and just keep the reference, if needed. same goes for bindings
% In practice, this MSD limitation can be mitigated if needed using a \textit{flexible algorithm}~\cite{I-D.ietf-lsr-flex-algo}, which allows the IGP to compute
% segments and shortest paths based on different metrics.
% % Flexible algorithm (Flex-Algo) allows the IGP to compute shortest paths based on metrics different from the IGP cost, \eg the delay. These can in turn also be translated in segments that can be encoded within the packet.
% Thus, one can not only use IGP-oriented segments but also delay-oriented segments (representing paths of lowest delay). %These new node segments %(\ie new edges in our multi-metric SR graph) can help to shift the general distribution observed in Fig.~\ref{fig:nbseg} to the left.
% Furthermore, outliers can be dealt with through \textit{binding segments}~\cite{RFC8402}, which create a mapping between a segment $b$ and a list of node or adjacency segments. Upon reading $b$, a router replaces it with the corresponding segment list. This allows to decrease the number of segments to stack at the edge router.

% In summary, while, in some rare cases, the MSD constraint may prevent the deployment of non dominated paths, this is not a real issue in practice. Nearly all DCLC solutions do not require more than 9 segments. % in all the cases.
% %On real topologies, DCLC paths require only few segments even when generalizing it to 2COP.
% For some corner-cases, SR can mitigate this theoretical limit
% by relying on flex-algo or binding segments.

% TODO: what's the point of best2cop then ?

% Only heterogeneous demands (with distinct constraints and less interesting objectives) can pose a rare issue with random weighted graphs. We finally argue that, if necessary, SR can mitigate this theoretical limit by relying on a flex-algo (or binding) control on the delay metric.


==> clean_latex/sections/best2cope.tex <==
\section{BEST2COP(E): Efficient Data Structures and Algorithms for Massive Scale Networks}\label{sec:best2cop}
%Leveraging Delay Measurements,

This section presents our contributions. We introduce and define preliminary notations and concepts used to design \bestcop,
before describing the data structures used by our algorithm.
In section \ref{sec:flat},  we describe our algorithm, \bestcop,
and show how we extend it for massive-scale networks divided in several areas in section~\ref{sec:areas}.
% We start with the SR Graph construct we rely on to then formally generalize the DCLC-SR problem with 2COP.
%  we briefly describe our algorithm, \bestcop, in its flat version, and show how we extend it for massive scale networks divided in several areas in section \ref{sec:areas}.
% Finally, we discuss the overall complexity of our approach along with the guarantees it provides.

We have shown that SR seems indeed appropriate (as desired) for fine-grained delay-based TE. We thus aim to solve DCLC in the context of an ISP deploying SR, leading to the DCLC-SR problem that considers the IGP cost, the propagation delay, and the number of segments.

For readability purposes, we denote:
\begin{itemize}
  \item $M_0$ the metric referring to the number of segments, with the constraint $c_0$ = MSD applied to it;
  \item $M_1$ the delay metric, with a constraint $c_1$;
  \item $M_2$ the IGP metric being optimized.
\end{itemize}

Given a source $s$, \textbf{DCLC-SR} consists in finding, for \textit{all} destinations, a \textit{segment list} verifying
two constraints, $c_0$ and $c_1$, respectively on
the number of segments ($M_0$) and the delay ($M_1$),
while optimizing the IGP distance ($M_2$). We denote this problem DCLC-SR$(s, c_0, c_1)$.
On Fig.~\ref{fig:DCLCGeant}, we would have DCLC-SR$(\mathit{Frankfurt}, 3, 8) \supset \mathit{Frankfurt}-\mathit{Budapest}-\mathit{Vienna}$. This DCLC path (shown in yellow in Fig~\ref{fig:DCLCGeant}), is indeed the best option to reach Vienna when considering an arbitrary delay constraint of 8ms. Since the best IGP path from Frankfurt to Vienna (the green one) does not go through Budapest, encoding this DCLC path requires at least one detour, i.e. one segment (here, a node segment instructing the packet to go through Budapest first).
% Note : since this is already somewhat said in the background, everything after
% "This DCLC paths ...." could be removed if needed


% (the yellow path made of one segment towards Budapest, which is the best option for the specific Vienna destination considering an arbitrary delay constraint of 8ms (the best IGP path towards Vienna being the green one, the DCLC path requires at least one detour, i.e. one segment).

% Before generalizing DCLC-SR in section \ref{sec:2cop} with 2COP (2 Constrained and 1 Optimal Path), let us first provide some context and properties we will rely on to efficiently solve such a problem.
To solve such a challenging problem, efficient data structures are required.
In the following, we first introduce the constructs we leverage and how we benefit from the inaccuracy of real delay measurements in particular.

\subsection{DCLC and True Measured Delays}\label{sec:true}
%The characteristics of real ISP networks can be leveraged to solve DCLC.


% pseudo-polynomial: as long as one of the two metrics is bounded, the exploration space is bounded as well.
\subsubsection{Leveraging measurement inaccuracy}
As mentioned, DCLC is weakly NP-Hard, and can be solved exactly in pseudo-polynomial time. In other words, as long as either the cost of the delay possesses only a limited number of distinct values (i.e., paths can only take a limited number of distinct distances),  the Pareto front of the paths' distances is naturally bounded in size as well, making DCLC tractable and efficiently solvable\footnote{Metric $M_0$ is omitted for now as this trivial distance is only required for SR and discussed in details later. While dealing with a three-dimensional Pareto front seems more complex at first glance, we will show that SR eventually reduces the exploration space because its operational constraint is very tight in practice and easy to handle efficiently.}.
Such a metric thus has to be bounded and possess a coarse accuracy (i.e., be discrete).
Although this has little impact when solving DCLC in a theoretical
context, it can be strongly leveraged to solve DCLC efficiently thanks to the characteristics of real ISP networks.


% The delay is nice
% This bounded metric can possess a coarse accuracy by nature, and/or its associated constraint can be small enough to sufficiently reduce the number of values within the solution space.
We argue that the metrics of real ISP networks do indeed possess a limited number of distinct values.
Although \bestcop can be adapted to fit any metric, we argue that $M_1$, the propagation delay, is the most appropriate one.
Indeed, IGP costs depend on each operators' configurations. For example, while some may rely on few spaced weights, others may possess intricate weight systems where small differences in weights may have an impact. Thus, bounding the size of the Pareto front based on the IGP costs is not only operator-dependant, but might still result in a very large front.


On the other hand, the delay (i) is likely strongly bounded,
and (ii) can be handled as if having a coarse accuracy in practice.
% will, by design and most of the time, have less distinct values than $M_2$ in the general case.
% Why is the delay nice ?
For TE paths, the delay constraint is likely to be very strict (10ms or less). Second, while the delay of a path is generally represented by a precise number in memory, the actual accuracy, \ie the trueness $t$ of the measured delay is much coarser due to technical challenges~\cite{RFC7679, RFC2681}.
In addition, delay constraints are usually formulated at the millisecond granularity with a tolerance margin, meaning that some loss of information is acceptable.
%ISPs are aware that measured delays are an estimation, not a guarantee.
% Propagation delays (usually measured with softwares like OWAMP~\cite{RFC4656}/TWAMP~\cite{RFC5357}) have limited accuracy, even with efficient hardware PTP time-stamping systems or accurate two-way delay link estimators. Due to both its inherent variation depending on physical properties, clock synchronization, or inconstant packet processing delays~\cite{RFC7679, RFC2681}, we argue that truly distinguishing the delay of a path at the granularity of the micro-second is very challenging.
%if not impossible nowadays in most ISPs.

Thus, floating numbers representing the delays can be truncated to integers, e.g., taking 0.1ms as unit.
%  to achieve a reasonable tradeoff regarding typical constraints between 1 and 10ms.
This allows to easily bound the number of possible non-dominated distances to $c_1 \times \gamma$, with $\gamma$ being the desired level of accuracy of $M_1$ (the inverse of the unit of the delay grain, here 0.1ms). %, and $c_1$ the delay constraint.
For example, with $c_1 = 100$ms and a delay grain of 0.1ms ($\gamma = \frac{1}{0.1} = 10$), we have only $1000$ distinct (truncated) non-dominated pairs of distances to track at worst. This leads to a predictable and bounded Pareto front.
One can then store non-dominated distances within a static array, indexed on the $M_1$-distance (as there can only be one non-dominated couple of distances $(M_1, M_2)$ for a given $M_1$-distance).
% For each truncated delay, it becomes then sufficient to store
% % only the best $M_2$-distance (indexed on its respective $M_1$-distance), leading to a predictable, reduced Pareto front that can be stored and managed in a static array.
% only the best $M_2$-distance (indexed on its respective $M_1$-distance), leading to a predictable, reduced Pareto front that can be stored and managed in
% a static array.

 In the remaining of the paper, $\Gamma$ denotes the size allocated in memory for this Pareto front array (i.e., $\Gamma = c_1 \times \gamma$). When $t$, i.e., the real level of accuracy, is lower (or equal) than $\gamma$, the stored delay can be considered to be exact. More precisely, it is discretized but with no loss of relevant information.
When $t$ is too high, one can choose $\gamma$ such that $\gamma < t$,
to keep $\Gamma$ at a manageable value. In this case, some relevant information can be lost, as the discretization is too coarse. While this sacrifices the exactitude of the solution
(to the advantage of computation time), our algorithm is still able to provide predictable guarantees
in such cases (\ie a bounded error margin on the delay constraint). This is further discussed in Section~\ref{sec:b2coplimits}.

% Otherwise, the correctness is no longer granted because one can opt for performance rather than increasing $\Gamma$ (to remain exact at the detriment of the efficiency); with such an option, our algorithm is nevertheless able to provide predictable guarantees, i.e. a bounded error margin on the delay constraint, discussed in details in section \ref{sec:b2coplimits}.
\red{\subsubsection{Fine, but which delay?}
Referring to a path's delay may be ambiguous. Indeed, this characteristic is not monolithic. The total delay is mainly composed of the propagation delay and the queuing delay. Both delays may play an important part in the overall latency, though none can be stated to be the main factor~\cite{end2end}. Although the propagation delay is stable, the queuing delay may vary depending on the traffic load. However, in order to compute TE paths, the delay metric must be advertised (usually within the IGP itself). For this reason, it is strongly recommended
to use a stable estimate of the delay, as varying delay estimations may lead to frequent re-computations, control-plane message exchanges, and fluctuating traffic distribution~\cite{RFC7471,RFC8570}.}

\red{For this reason, we use the propagation delay, as recommended in ~\cite{RFC7471,RFC8570}. The latter is usually measured through the use of a priority queue, ignoring so the queuing delay. Its value is deduced as a minimum from a sampling window, increasing so its stability~\cite{perfmes}. Using this delay not only makes our solution practical (as we rely on existing measurements and respect protocol-related constraints), but is actually pertinent in our case. In practice, flows benefitting from DCLC paths benefit from a queue with high priority and experience negligible queueing delays. In addition, the amount of traffic generated by such premium interactive flows can be controlled to remain small enough if it is not limited by design. Consequently, not only is there no competition between premium flows and best-effort traffic, but these flows do not generate enough traffic to lead to significant competition between themselves. Thus, the experienced delay is actually agnostic of the traffic load for our use-case, making the propagation delay a relevant estimate.
Consequently, we use the discretized propagation delay, enabling both practical deployment and the limitation of the number of non-dominated distances, within our structure used to encompass Segment Routing natively, the SR graph.
}

\subsection{The SR Graph and 2COP}\label{sec:sr-graph}

%We here show how we reflect both the properties on our specific construct used to encompass SR and the two metrics, to
To solve DCLC-SR efficiently, as well as its comprehensive generalization, 2COP, we rely on a specific construct used to encompass SR, the delay, and the IGP cost: the \textit{multi-metric SR graph}.
%We then present and briefly illustrate 2COP, a comprehensive generalization of DCLC-SR.% in Sec.~\ref{sec:2cop}.

\subsubsection{Turning the Physical Graph into a Native SR Representation}
\label{ssec:srgraph}
% What's the SR Graph ?
This construct represents the segments as edges to natively deal with the $M_0$ metric and its constraint, $c_0=\text{MSD}$.
The valuation of each edge depends on the distance of the path encoded by each segment.
%whose weights are equal to the weights of the path encoded by the segment,
While the weights of an adjacency segment are the weights of its associated local link, the weights of a node segment are the distances of the ECMP paths it encodes: the \red{(equal) IGP cost (\ie, M2-distance)}, and the lowest guaranteed delay (\ie, the M1-distance), \ie the worst delay among all ECMP paths.
Hence, computing paths on the SR graph is equivalent to combining stacks of segments (and the physical paths they encode), as stacks requiring $x$ segments are represented as paths of $x$ edges in the SR graph (agnostically to its actual length in the raw graph).
The SR graph can be built for all sources and destinations thanks to an All Pair Shortest Path (APSP) algorithm.
% to deduce the weight of each node segment.
Note that this transformation is inherent to SR and leads to a complexity of $O(n (n\log(n) + m))$, for a raw graph having $n$ nodes and $m$ edges, with the best-known algorithms and data structures. This transformation (or rather, the underlying APSP computation) being required for any network deploying TE with SR (the complexity added by our multi-metric extension being
negligible), we do not consider it as part of our algorithm presented later.% of take it into account when evaluating ,
% whose complexity will not exceed the one just mentioned.

% Notations
%Fig.~\ref{fig:exampleraw}, which depicts an arbitrary raw graph,
This transformation is shown in Fig.~\ref{fig:examplesr}, which shows the SR counterpart of the raw graph provided in Fig.~\ref{fig:DCLCGeant}.
To describe this transformation more formally, let us denote $G = (V, E)$ the original graph, where $V$ and $E$ respectively refer to the set of vertices and edges. As $G$ can have multiple parallel links between a
pair of nodes $(u,v)$, we use $E(u,v)$ to denote all the direct links between
nodes $u$ and $v$.
% When necessary, we denote a specific link $(u_x, v)$, $x$
% specifying the considered interface.
Each link $(u,v)$ possesses two weights, its delay $w_1^{G}((u,v))$ and its IGP cost $w_2^{G}((u,v))$.
The delay and the IGP cost being additive metrics, the $M_1$ and $M_2$ distances of a path $p$ (denoted $d_1^G(p)$ and $d_2^G(p)$ respectively) are the sums of the weights of its edges.

From $G$, we create a transformed multigraph, the SR graph denoted $G' = (V,
E')$. While the set of nodes in $G'$ is the same as in $G$, the set of edges
differs because $E'$ encodes segments as edges representing either adjacency or node segments encoding respectively local physical link or sets of best IGP paths (with ECMP).
%We use similar notations for $G'$.
The $M_i$-weight of an edge in $G'$ is denoted $w_i^{G'}((u,v))$.
%for node segments, and $w_i^{G'}((u_x,v))$ for adjacency segments.
However, to alleviate further notations, we denote simply $d_i(p)$ the $M_i$ distance of a path in $G'$ instead of $d_i^{G'}(p)$.
Note that if $G$ is connected, then $G'$ is a complete graph thanks to node segments.


\red{\textbf{SR graph: Node segment encoding.}} A node segment, encoding the whole set $P_G(u,v)$ of ECMP best paths
between two nodes $u$ and $v$, is represented by exactly one edge in $E'(u,v)$. The $M_2$-weight $w_2^{G'}((u,v))$ of a node segment is the (equal) $M_2$-distance of $P_G(u,v)$.
Since, when using a node segment, packets may follow any of the ECMP paths,
we can only guarantee that the delay of the path will not exceed the
maximal delay out of all ECMP paths. Consequently, its $M_1$-weight $w_1^{G'}((u,v))$ is defined as the maximum $M_1$-distance among all the paths in $P_G(u,v)$.
Links representing node segments in $G'$ thus verify the following:
\[
\begin{array}{l}
    w_1^{G'}((u,v)) = \max_{p\in P_G(u,v)} d_1^G(p)\\
    w_2^{G'}((u,v)) = d_2^G(p)\quad \text{for any }p\in P_G(u,v)
\end{array}
\]

\red{\textbf{SR graph: Adjacency segment encoding.}} An adjacency segment corresponds to a link in the graph $G$ and is represented by an edge $(u_x,v)$ in $E'(u,v)$,
whose weights are the ones of its corresponding link in $G$, only if it is not dominated by the node segment $(u,v)_{G'}$ for the same pair of nodes, \ie if
$w_1^{G'}((u,v)) > w_1^{G}((u_x,v))$, or by any other non-dominated adjacency
segments $(u_y,v)$, \ie if $w_1^G((u_y,v)) > w_1^{G}((u_x,v))$ or
$w_2^G((u_y,v)) > w_2^{G}((u_x,v))$, where $(u_x, v)$ and $(u_y, v)$ are two different outgoing links of $u$ in $E(u,v)$\footnote{If two links have exactly the same weights, we only add one adjacency segment in $G'$}.\\

Fig.~\ref{fig:examplesr} illustrates the result of such a transformation: one can easily identify the three non-dominated paths between Frankfurt and Vienna, bearing the same colors as in Fig.~\ref{fig:DCLCGeant}.
The green path (\ie the best $M_2$ path) is encoded by a single node segment. The pink, direct path (\ie the best $M_1$ path) is encoded by an adjacency segment (the double line in Fig.~\ref{fig:examplesr}).
The yellow paths (the solution of DCLC-SR(Frankfurt, 3, 8) and an interesting tradeoff between $M_1$ and $M_2$) requires
an additional segment, in order to be routed through Budapest.
Note that in practice, the last segment is unnecessary if it is a node segment, as the packet will be routed towards its final IP destination through the best $M_2$ paths natively.


% , the second (pink double line) uses an adjacency segment (the best $M_1$ path), while the last yellow (dotted) one requires one additional segment via Budapest but represents an interesting tradeoff between $M_1$ and $M_2$.
% \QB{j'ai ajouté dotted et dashed dans le cas d'une impression noir et blanc mais ça fait un peu lourd du coup (a changer sur la figure si on le garde)}

% %$(u_x, v)$
% %($w_1^{G'}((u_x,v))$, $w_2^{G'}((u_x,v))$)
% Such an adjacency is represented by an edge

% Fig.~\ref{fig:exampleraw} exhibits two paths from $r$ to $q$ in $G$ which have an optimal IGP-cost of
% 8: $(r,q)$ with distance $(1.11 ; 8)$ and
% $\makepath{{(r_1,o)}, {(o, p)}, {(p,q)}}$ with distances $(4.69 ; 8)$. These ECMP paths are represented by the unique link $(r,q)_{G'}$, a node segment (in plain black in $G'$), with the rounded\footnote{Using \textit{true delays}, \ie M$_1$ weights rounded to integers to take advantage of the limited accuracy of the delay measurement, greatly reduce the complexity of the problem if Pareto front updates are limited to distinguishable values.} distance $(47 ; 8)$. % while remaining exact.
% However, using an adjacency segment to enforce the direct link between $r$ and $q$ offers a better delay (1.11 vs 4.7). Thus, since it is not dominated, we add the adjacency segment $(r_1,q)$ with distances $(11 ; 8)$ to the SR Graph.


% \begin{figure}
%   \centering
%   \includegraphics[scale=0.7]{exraw-new.pdf}
%   \caption{The raw network graph $G = (V,E)$ is a multigraph, with weighted edges.
%   The weight of the edges is represented as a couple (delay;IGP cost). While there
%   sometimes only exist a single edges between two nodes, such as $(s,r)$, we otherwise distinguish between parallel nodes such as $(s_1,n)$ and $(s_2, n)$.}
%   \label{fig:exampleraw}
% \end{figure}


\begin{figure}
  \centering
  \includegraphics[scale=0.5]{GEANTSR_disc.pdf}
  \caption{
  This Figure shows the network from Fig.~\ref{fig:DCLCGeant} translated into an SR graph.
  The SR graph encodes segments as edges. Plain edges represent node segments, \ie sets of ECMP paths. Double-lines are adjacency segments, here only $(\mathit{Frankfurt},\mathit{Vienna})$, and are visible only if they are not dominated by other segments. Colored edges refer to the paths highlighted in Fig.~\ref{fig:DCLCGeant}.}
  %, making $G'$ a full-mesh at least.
  \label{fig:examplesr}
\end{figure}



\red{Our multi-metric SR graph (or equivalent constructs gathering the multi-metric all-pair shortest path data) is mandatory to easily consider the number of segments necessary to encode the paths being explored. However, its usage can differ in practice. We envision two modes which allow to consider this additional "off the graph" metric, using our SR Graph.}\\



\red{\textbf{Using the SR Graph to perform path conversions.} One of the two options is to run the path computation algorithm on the original topology, and convert the paths being explored to segment lists. Performing this conversion is however not trivial. One must return the minimal encoding of the given path (with respect to the number of segments) while correctly managing the (forced) path diversity brought by ECMP, which may exhibit heterogeneous delays. However, one can efficiently perform such conversion when relying on our SR graph. By
summarizing the relevant information (\ie the worst-case delay within ECMP paths), the SR Graph allows to easily consider the ECMP nature of SR within a multi-metric context. %\footnote{Note that the APSP data may be store differently and still allow for efficient conversion. However, we argue that the SR graph allows for an efficient storage of such data memory-wise.}. 
However, the segment metric $M_0$ is peculiar. Extending a path does not always imply an increase in the number of necessary segments. Furthermore, the number of segments required to encode two distinct paths may evolve differently, even when the latter are extended from the same node with the same edge. Because of these properties, the way to check paths for dominancy must be revised. This extended dominance check may lead to an increased number of paths to extend, and thus to a higher worst-case complexity. Further details regarding the conversion algorithm and the extended dominancy check can be found in ~\ref{app:LCA}.}\\


\red{\textbf{Using the SR Graph natively.} Another method is to run the path computation algorithm directly on the SR graph we described. 
Note that this forces the algorithm to run on a complete graph, which may significantly increase the overall complexity. However, the segment metric $M_0$, originally an "off the graph" metric with singular properties, becomes a standard graph metric, as it is now expressed by the number of edges that compose the paths (a path encoded by $x$ segments has $x$ edges within the SR Graph). This method also allows using standard, known algorithms as-is to solve the DCLC-SR problem.\\}


\red{When designing our algorithm, \bestcop, we use the second approach. Indeed, by using a bellman-ford-like exploration of the SR Graph, one can not only easily prune paths requiring more than $MSD$ segments, but also benefit from efficient Pareto front management and multi-threading. These various features allow \bestcop to efficiently solve not only DCLC-SR, but also 2COP, a more general and practically relevant problem regarding the computation of constrained paths within an SR domain. Note, however, that we will provide our competitor with both approaches to make the evaluation as fair as possible.}

% \red{While we chose to use the SR Graph natively with \bestcop, we compare ourselves to two versions of our competitor, using both approaches, to make the evaluation as fair as possible.



% We implement such an approach able to efficiently handle all this aspects (on the fly at each path extension without redundant computations) and verify its correctness by ensuring the same outcome as the native SR graph usage. In the evaluation section, we will discuss and compare both approaches according to the underlying graph characteristics (e.g., its density and its multi-weights setting).




\subsubsection{The 2COP Problem(s)}
\label{sec:2cop}
%This section introduces 2COP, a generalization of DCLC-SR.
Solving DCLC-SR exactly requires, by definition, to visit the entirety of the Pareto front for all destinations.
However, although only some of these paths are DCLC-SR solutions for a given delay constraint, all paths visited during this exploration may be of some practical interest. In particular, some of them solve problems similar to DCLC but with different optimization strategies and constraints. By simply memorizing the explored paths (\ie storing the whole Pareto front within an efficient structure), one can solve a collection of practically relevant problems. For instance, one may want to obtain a segment path that minimizes the delay, another the IGP-cost, or the number of segments. Solving 2COP consists in finding, for all destinations, paths optimizing all three metrics independently, and respecting the given constraints.
%, which encompass all these latter.
We formalize this collection of problems as 2COP.
Solving 2COP enables more versatility in terms of optimization strategies and handles heterogeneous constraints for different destinations.
Simply put, while DCLC-SR is a one-to-many DCLC variant taking MSD into account, 2COP is more general as it includes all optimization variants.

% NOTE FIRST REVISION COMNET:
% JRO; I removed everything here but we may want to put it back
% With 2COP, one can also actually claim to be highly flexible regarding constraints (and optimization strategies). Besides the three optimization variants, other practically relevant heterogeneous problems can be solved.
% In practice, a customer may change its needs after the execution of our algorithm. In particular, one may wish for a smaller constraint if some requirements become stricter. Finally, ISPs could be interested in finding destination-specific constraints and optimizations, \ie different constraints and strategies for each destination.
% While algorithms returning only DCLC-SR solutions would have to be run multiple times and re-calibrated to solve the situations mentioned above (different optimization strategies, stricter constraints, or destination-specific constraints), our algorithm returns the whole Pareto Front.

With initial constraints $c_0, c_1, c_2$, \bestcop solves 2COP, \ie returns in a single run paths that satisfy smaller constraints $c_0', c_1', c_2'$ for any $c_i' < c_i$, $i = 0,1,2$, \red{offering more flexibility than simply returning the DCLC-SR solution}.
% Basically, \bestcop returns and structures the entire constraint Pareto front to solve the 2COP problem in a very general way, and thus does not need to be re-run to find stricter constrained paths optimizing other metrics.
%More formally,

\textbf{Definition.}
  \textit{\textbf{2-Constrained Optimal Paths (2COP)}\\
  Let $f(M_j, c_0, c_1, c_2, s, d)$ be a function that returns a feasible segment path from s to d (if it exists),
  verifying all constraints $c_i, 0 \leq i \leq 2$ and optimizing $M_j,j \in {0,1,2}$. For a given source $s$ and given upper constraints $c_0, c_1, c_2$, we have}
   \begin{gather*} 2COP(s, c_0, c_1, c_2) =
   \bigcup_{\substack{
    \forall d \in V,\\
    \forall j \in \{0,1,2\},\\
    \forall c_j' \leq c_j
          }}
   f(M_j, c_0', c_1', c_2', s, d)
   \end{gather*}

%\hfill$\blacksquare$
Observe that, for any $s \in V$, DCLC-SR($s, c_0, c_1$) consists of the paths in $2COP(s, c_0, c_1, \infty)$ minimizing $M_2$.
Looking at Fig.~\ref{fig:examplesr}, we have two interesting examples (we rely on the first capital letter of the cities):
 \begin{gather*}
  f(M_2,3,70,\infty,F,V) = \makesrpath{{(F,B)}, {(B,V)}}~(67,4)\\
  %f(M_1,3,\infty,\infty,M,B) = \makesrpath{{(M,V)}, {(V,M)}}~(60,3)\\
  %f(M_1,3,\infty,\infty,G,B) = \{\makesrpath{{(G,M)}, {(M,V)}, {(V,B)}}~(77,4)\\
  f(M_1,3,\Gamma,\infty,G,B) = \makesrpath{{(G,M)}, {(M,B)}}~(77,4)
 \end{gather*}
%
%
% Let us use Fig.~\ref{fig:examplesr} to illustrate the most basic 2COP features.
% In this graph, we have
% \begin{gather*}
% f(M_1,3,70,\infty,s,p) = \makesrpath{{(s,r)}, {(r_1,q)},{(q,p)}}~(34,14)\\
% f(M_2,3,70,\infty,s,p) = \makesrpath{{(s_1,n)}, {(n,o)},{(o,p)}}~(65,4)
% \end{gather*}
%
% Notice that the segment path $\makesrpath{{(s,n)},{(n,o)},{(o,p)}}~(66,4)$ is also optimal for $M_2$ while respecting $c_1$, but it is dominated by $\makesrpath{{(s_1,n)},{(n,o)},{(o,p)}}~(65,4)$, hence only the non-dominated solution is considered.
% Also, observe that the path minimizing $M_1$ is here different from the one minimizing $M_2$.
% Our algorithm is able to return both of these solutions in a single run.
%
% Referring again to Fig.~\ref{fig:examplesr},
% and restricting the set of solutions to paths towards destination $p$ only, we have
% \begin{gather*}
% \text{2COP}(s, 3, 70, \infty) = \{\makesrpath{{(s,r)},{(r,p)}}~(46,6),\\ \makesrpath{{(s_1,n)}, {(n,o)} ,{(o,p)}}~(65,4),
%  \makesrpath{{(s,r)}, {(r_1,q)} ,{(q,p)}}~(34,14),\\ \makesrpath{{(s_1,n)},{(n_1,o)},{(o,p)}}~(64,5)\}
% \end{gather*}
%
% Thus, all the solutions minimizing $M_1$, $M_2$ or $M_0$ are already present in the 2COP set.
% For example, the path respecting the constraints and minimizing $M_2$ is $f(M_2, 3, 70, \infty, s, p) = \makesrpath{{(s_1,n)}, {(n,o)} ,{(o,p)}}~(65,4)$ while if one prefers to minimize $M_0$ it can rely on $\makesrpath{{(s,r)},{(r,p)}} = f(M_0,\infty, 64, \infty,s,p)$.
% In addition, to enforce a stricter constraint a posteriori, \eg $c_1 = 64$ instead of 70, the new results can also be found in the 2COP output without re-running the algorithm. The new result would be here $f(M_1, 3, 64, \infty,s,p) = \makesrpath{{(s_1,n)},{(n_1,o)},{(o,p)}}~(64,5)$.
In the second example, recall that the M1-distances are truncated to obtain integer values and $\Gamma$ is the maximum $c_1$ constraint we consider (multiplied by $\gamma$).

When the delay accuracy allows to reduce the problem's complexity sufficiently, \bestcop can solve exactly any of the variants within 2COP \red{and return any desired output of the image of $f$}.

% FIRST REVISION: removed this as well.
% Our algorithm, \bestcop takes the constraints and the SR graph $G'$ as inputs and builds in polynomial time an array that can return any desired output of the image of $f$ given stricter sub-constraints instead of relaunching the algorithm. Retrieving the desired output can be performed in constant (or at worst sub-linear) time.

In Sec.~\ref{sec:b2coplimits}, we detail how we can handle each 2COP variant with guarantees when the delay accuracy is too high to provide exact solutions while remaining efficient.
Solving 2COP can be implemented as efficiently as solving only DCLC-SR.

\subsection{Our Core Algorithm for Flat Networks}
\label{sec:flat}

In this section, we describe \bestcop, our algorithm efficiently solving 2COP (and so DCLC-SR).
% by leveraging properties formalized in the previous section.
Its implementation is available online\footnote{\url{https://github.com/talfroy/BEST2COP}}.
\red{Although \bestcop was already described in our previous contribution, a complete and far more detailed algorithmic description can be found in ~\ref{app:b2cop} for the interested reader.}

Akin to the SR graph computation, \bestcop can be run on a centralized controller but also by each router.
Its design is centered around two properties.
First, the graph exploration is performed so that paths requiring $i$ node segments are found at the $i^{\mathit{th}}+1$ iteration\footnote{Note that each adjacency segment translates to at least one necessary segment, two if they are not globally advertised and not subsequent.}, to natively tackle the MSD constraint.
Second, \bestcop's structure is easily parallelizable, allowing to benefit from multi-core architectures with low overhead.

\red{Simply put, at each iteration, \bestcop starts by extending the known paths by one segment (one edge in the SR graph) in a Bellman-Ford fashion (a not-in-place version to be accurate). Paths found during a given iteration are only checked loosely (and efficiently) for dominancy at first. This extension is performed in a parallel-friendly fashion that prevents data-races, allowing to easily parallelize our algorithm. \red{Only once} at the end of an iteration are the newly found paths filtered and thoroughly checked for dominancy, to reflect the new Pareto front. The remaining non-dominated paths are in turn extended at the next iteration. %themselves.
These steps only need to be performed $MSD \approx 10$ times, ignoring so all paths that are not deployable through SR.}
When our algorithm terminates, the results structure contains, for each segment number, all the distances of non dominated paths from the source towards all destinations.
\red{The interested reader may find further details regarding how 2COP solutions are extracted from the results structure in  Appendix~\ref{sec:best2cop}.}

%All paths not explored before the tenth iteration can be ignored as they require more than MSD segments.

\red{The good performance of \bestcop comes from several aspects. First, the fact that paths requiring more than MSD segments are natively excluded from the exploration space. Second, well-chosen data structures benefiting from the
limited accuracy of the delay measurements to limit the number of paths to extend. This allows to
manipulate arrays of fixed size, because the Pareto front of distances towards each node is limited to $\Gamma$ at each step (enabling very efficient read/write operations). Third, using a Bellman-Ford approach allows not only to easily parallelize our algorithm but also to perform lazy efficient update of the Pareto front. Indeed, a newly found path may only be extended at the \textit{next} iteration. Thus, we can efficiently extract the non-dominated paths from all paths discovered during the current iteration in a \text{single} pass, once at the end of the iteration. Conversely, other algorithms
tend to either check for dominancy whenever a path is discovered
(as the later may be re-extended immediately), or not bother to check for dominancy at all, \eg by relying solely on interval partitioning to limit the number of paths to extend.}
%JRO TODO CHECK THIS


% These simple data structures, frequently used for read/write operations, allow for updating Pareto fronts very efficiently with an amortized relaxation cost (conversely to priority queues with Dijkstra-like algorithms).
% Using a Bellman-Ford approach thus comes with two advantages: straight-forward parallelism and lazy updates of the Pareto fronts.

 % (\ie storing the predecessor every time we insert an element in the Pareto front). With this structure, one can easily obtain a path associated with a given distance in the Pareto front, like it is usually done with the Dijkstra Algorithm.
% In addition, one could also list all possible paths associated with a given distance in the Pareto front using the structure \varpfront only, by backward induction (even if each possible path can be computed in a polynomial time, recall that there may be an exponential number of such paths).



\subsection{For Massive Scale, Multi-Area Networks}
\label{sec:areas}

As shown in~\cite{nca2020}, this algorithms exhibits great performance on large-scale networks of up to \num{1000} nodes ($\approx 15$ms).
However, since the design of \bestcop implies a dominant factor of $|V|^2$ in term of time complexity\footnote{The detailed complexity is given in section \ref{sec:complexitybis}} (the SR graph being complete), recent SR deployments with more than $\num{10000}$ nodes would not scale well enough.
The sheer scale of such networks, coupled with the inherent complexity of TE-related problems, makes
2COP very challenging if not impossible to practically compute at first glance.
In fact, even \bestcop originally exceeds 20s when dealing with $\approx$\num{15000} nodes.
As we will see in the evaluations, this is much worse with concurrent options.

In this section, we extend \bestcop in order to deal efficiently with massive scale networks.
By leveraging the physical and logical partitioning usually performed in such networks, we manage to solve 2COP in $\approx 1$s even in networks of \num{100000} nodes.

\subsubsection{Scalabity in Massive Network \& Area decomposition}
The scalability issues in large-scale networks do not arise solely
when dealing with TE-related problems. Standard intra-domain routing protocols encounter issues past several thousands of nodes. Naive network design creates a large, unique failure domain resulting in numerous computations and message exchanges, as well as tedious management.
Consequently, networks are usually divided, both logically and physically, in \textit{areas}.
This notion exists in both major intra-domain routing protocols (OSPF and IS-IS). In the following, we consider the standard OSPF architecture and terminology but our solution can be adapted to fit any one of them

Areas can be seen as small, independent sub-networks (usually of around 100 - 1000 nodes at most). Within OSPF,
routers within an area maintain a comprehensive topological database of their own area only. Stub-areas are centered around the \textit{backbone}, or area 0. \textit{Area Border Routers}, or ABRs, possess an interface in both the backbone area and a stub area. Being at the intersection of two areas, they are in charge of sending a summary of the topological database (the best distance to each node) of one area to the other. There are usually at least two ABRs between two areas. We here (and in the evaluation) consider two ABRs, but the computations performed can be easily extended to manage more ABRs.
Summaries of a non-backbone area are sent through the backbone. Upon reception, ABRs inject the summary within their own area. In the end, all routers possess a detailed topological database of their own area and the best distances towards destinations outside of their own area.
% Not only does this reduces the computation cost induced in each area, but only specific destinations could be advertised between areas (e.g. stub sub-networks but not transit ones) to mitigate the overall churn and overhead to $\approx |V|$ distances.
% JRO: instead of |E| ? Si nous on s'est gouré sur le fait que un lien = une destination,
% peut être que ça va pas être évident pour le lecteur que avec des aires c'est pas
% V de base

%This reduces the number of entries to manage (scaling with the number of nodes $|V|$ rather than the number of edges $|E|$) as well as the scale of the failure domain.


\subsubsection{Leveraging Area Decomposition}
% This area-decomposition can (and should) be leveraged by TE
% algorithms in order to deal with massive scale networks.

This partitioning creates obvious separators within the graph, the ABRs. Thanks to the latter, we can leverage this native partition in a \red{similar} divide-and-conquer approach, adapted to the computation of 2COP paths, by running \bestcop at the scale of the areas before exchanging and combining the results.
We do not only aim to reduce computation time, but also to keep the number and size of the exchanged messages manageable.

%Before discussing our design in detail, we start with a high-level description of the way we extend \bestcop:

% FIRST REVISION: removed all the enumerate
% \begin{enumerate}
%   \item Routers compute the multi-metric SR graph of their \textit{own areas}, before running \bestcop on the resulting area-SR-graph. Note that ABRs, being adjacent to two areas, should run \bestcop twice;
%   \item ABRs share their \red{results}, that is all non-dominated distances, and their segment lists, towards destinations within their own area;
%   \item ABRs now possess all non-dominated paths to others ABRs (from running \bestcop on area 0) and all non-dominated paths from these distant ABRs to the destinations in their corresponding areas (through message exchange). By combining both paths through a simple cartesian product and a light post-processing, one can get all 2COP paths to the destinations within distant areas.
%   %These paths may then be sent to routers within the local area, which in turn perform a similar processing.
% \end{enumerate}


We now explain how we perform this computation in detail.
For readability purposes, we rely on the following notations:
$\mathcal{A}_x$ denotes area $x$.
$A_x$ denotes the ABR between the backbone and $\mathcal{A}_x$.
When necessary, we may distinguish the two ABR $A1_x$ and $A2_x$. Finally, b2cop($\mathcal{A}_x, s, d$) denotes the results (the non-dominated paths) from $s$ to $d$ within $\mathcal{A}_x$.
When $d$ is omitted, we consider all routers within $\mathcal{A}_x$ as destination. Figure~\ref{fig:cartesian product} illustrates a network with three areas, $x$, $y$ and 0, the backbone area.\\
\red{We here chose to detail a simple distributed and router-centric variant of our solution.
%, where each router performs its own computations within its area and combines it with the distances advertised by the two ABRs of its area.
However, our solution may well be deployed in other ways, e.g. relying on controllers, or even a single one.
In such cases, the computation could be parallelized per area if needed. Such discussion is left for future work.\\}
% We can see that a non-dominated path from $s$ to $d$ is obtained by concatenating a non-dominated path in each area. Thus, the set of solutions is the cartesian product of the sets of solutions in each area.\\

% \textbf{Area-scale SR Graph.}
%  When a network grow in size, the computation
% of the SR graph (inherent to SR) becomes too complex.
 %, but only of they own area.
%In addition, this computation (inherent to SR) does not scale well.
%Thus, we compute the SR graph at the area scale.


\begin{figure}\centering
  \begin{tikzpicture}[
    router/.style={black,fill, circle, inner sep=0.04cm}
  ]
    \definecolor{airecolor}{rgb}{0.9,0.9,0.9}
    \fill[airecolor] (0,0) circle (0.8);
    \fill[airecolor] (180-20:1.6) circle (0.8);
    \fill[airecolor] (20:1.6) circle (0.8);
    \node[] (AireX) at (180-55:1.7) {$\mathcal{A}_x$};
    \node[] (AireY) at (55:1.7) {$\mathcal{A}_y$};
    \node[] (Aire0) at (90:.9) {$\mathcal{A}_0$};

    \node[router,label={180:$s$}] (s) at (180-20:2) {};
    \node[router,label={-135:$A_x$}] (A1) at (180-20:0.8) {};
    \node[router,label={-45:$A_y$}] (A2) at (20:0.8) {};
    \node[router,label={0:$d$}] (d) at (20:2) {};

    \draw (s) edge[bend left=15] (A1);
    \draw (s) edge[bend left=40] (A1);
    \draw (s) edge[bend right=15] (A1);
    \draw (s) edge[bend right=40] (A1);


    \draw (A1) edge[bend left=10] (A2);
    \draw (A1) edge[bend right=70] (A2);
    \draw (A1) edge[bend right=15] (A2);
    \draw (A1) edge[bend right=40] (A2);

    \draw (A2) edge[bend left=15] (d);
    \draw (A2) edge[bend left=40] (d);
    \draw (A2) edge[bend right=15] (d);
    \draw (A2) edge[bend right=40] (d);


    \node[black, circle, draw, fill=airecolor, inner sep=0.25] (B1) at (180-20:1.4) {$B_1$};
    \node[black, circle, draw, fill=airecolor, inner sep=0.45] (B1) at (90:.09) {$B_2$};
    \node[black, circle, draw, fill=airecolor, inner sep=0.25] (B1) at (20:1.4) {$B_3$};


    \node[] (Aire0) at (-90:1.1) {b2cop$(s,d) \subset B_1\times B_2 \times B_3$};
  \end{tikzpicture}
  \caption{The set of solutions across areas is obtained from the cartesian product of the solutions in each area.}\label{fig:cartesian product}
\end{figure}

% JRO: pas super content des 2/3 par suivant
\textbf{Working at area scale.}
\red{Due to the area decomposition, routers do not possess the topological information to compute a full, complete SR graph of the whole network. Thus, we make routers only compute the SR graph of their own area(s).}
%Once computed, it is tempting to make routers exchange the SR graph of their area,
%and run \bestcop on the union of all area-SR-Graphs.
%However, it systematically implies a large volume of information to share between areas.
\red{Because exchanging the SR graphs themselves implies a large volume of information to share, we instead make the ABRs exchange their 2COP paths (i.e., the non dominated paths to all destinations of their areas)}  %We claim that only sharing the Pareto fronts waste much less computing and message resource in practice
since we limit their numbers to $\Gamma$ at worst. This exchange still provides enough information for all routers to compute all 2COP paths for every destination.% within the network.}
% Relying on the fact that Pareto fronts of each destination are small enough in practice (lower than the full or even per-area SR-graph information), we
% argue that the latter provide the minimal necessary information to retrieve all 2COP paths among areas.

% We claim that only sharing the Pareto fronts of each destination for computing 2COP is useful will waste much less computing and message resource in practice since we limit their sizes to $\Gamma$ at wo
% Relying on the fact that Pareto fronts of each destination are small enough in practice (lower than the full or even per-area SR-graph information), we
% argue that the latter provide the minimal necessary information to retrieve all 2COP paths among areas

%(leading to a churn of $\approx \Gamma \times |V|$ instead of at worst $\approx |V|^2$)

%By merging then into a single graph, routers could theoretically
%compute 2COP paths thanks to \bestcop. However, due to the graph not being fully-meshed, the segment list deduced for each path may contain some (correctable) anomalies. Furthermore, exchanging the SR graph would result in a message complexity of $|V|^2$ at least.

%Thus, we chose instead to run \bestcop within each areas, before exchanging the non-dominated distances.
More formally, each ABR $A_x$ computes b2cop($\mathcal{A}_x, A_x$) and exchange the results with $A_y, \forall y \neq x$.
Areas being limited to a few hundreds routers on average, this computation is very efficient.
Note that ABRs also compute b2cop($\mathcal{A}_0, A_x$), but need not exchange it, as all ABRs perform this computation.
Exchanging the computed 3D Pareto front has a message complexity of $|V| \times c_0 \times \Gamma$ at worst in theory.
In practice, we expect both the size of Pareto fronts and the number of relevant destinations to consider to be fairly low ($<< \Gamma$ and $<< |V|$ resp.).
In the case of non-scalable Pareto fronts, one can opt for sending only part of them but at the cost of relaxing the guarantees brought by \bestcop.
% dire qu'on le mesure à 10
% pour 45000 noeuds ?
%Should the sent sample not be sufficient to compute the requested constrained path, the concerned node may ask explicitly for the detailed results.

After exchanging messages, any ABR $A_x$ should know the
non-dominated paths from itself to $A_y, \forall y \neq x$, and the non-dominated paths from $A_y$ to all nodes within $\mathcal{A}_y$. By combining this information, we can compute the non-dominated paths from $A_x$ to
all nodes within  $\mathcal{A}_y$, as we will now detail.\\

% b2cop($\mathcal{A_0}, A_x$) and b2cop($\mathcal{A_x}, A_x$)  from local computation, and b2cop($\mathcal{A_y}, A_y$) $\forall y \neq x$ from message exchange. Knowing t

% In conclusion, running \bestcop for a given  before sending the computed Pareto front to other ABRs allows to greatly reduce the message complexity (which becomes tunable) while staying true to the original intent between areas.

\textbf{Cartesian product.} Since ABRs act as separators within the graph, to reach a node within a given area $\mathcal{A}_y$, it is necessary to go through one of the corresponding ABRs $A_y$.
%This observation allows to easily compute non-dominated paths towards all nodes, once the Pareto fronts are exchanged. %Indeed,
It thus implies that non-dominated paths to nodes within $\mathcal{A}_y$ from
$A_x$ can be found by combining bcop($\mathcal{A}_0, A_x, A_y$) with bcop($\mathcal{A}_y, A_y$).
In other words, by combining, with a simple cartesian product, the local non-dominated paths towards the ABRs of a given zone with the non-dominated paths from said ABRs to nodes within the corresponding distant areas, one obtains a superset of the non-dominated paths towards the destinations of the distant area. In practice, since several ABR can co-exist,
% (typically two) bcop($\mathcal{A}_y, A1_y$) and bcop($\mathcal{A}_y, A2_y$),
it is necessary to handle the respective non-dominated paths (bcop($\mathcal{A}_y, A1_y$) and bcop($\mathcal{A}_y, A2_y$)) with careful comparisons to avoid incorrect combinations.\\
%merging them before performing the product,
%although it may be performed iteratively. However, the computed paths
%may not form a Pareto front, and may also contain some anomalies.\\


\textbf{Post-processing and merging.} To ensure that the results obtained through the cartesian product aforementioned are correct, some post-processing is required.
% More precisely, this post-processing allows to remove unnecessary segments for the segments lists, and to remove non-dominated paths from the computed cartesian product.
% First, the segment list associated with each path should be corrected.
When combining segment lists, the latter are simply concatenated.
%, the first sub-path thus always reaching an ABR.
More precisely, the resulting segment list necessarily possesses the following structure:
\makesrpath{{(u_0,u_1)}, \dots, {(u_i, A)}, {(A, v_0)}, \dots, {(v_{j-1}, v_j)}}, with $A$ denoting an ABR.
However, $A$ being a separator, it is likely that the best IGP path from $u_i$ to $v_0$ natively goes through $A$ without the need of an intermediary segment.
Thus, segments of the form \makesrpath{{(u_i, A)}, {(A, v_0)},} can often be replaced by a single segment $(u_i, v_0)$.
%\makesrpath{{(A_{-1}, A_{+1})},{}}.
Such anomalies should be corrected, as an additional useless segment may render the path falsely unfeasible, even though it actually fits the MSD constraint.
This correction can be performed easily.
Let $A1$ be the separator, if $(u_i, A1)$ and $(A1, v_0)$ are
node segments, and all best IGP paths from $u_i$ to $v_0$ go through $A1$ (or possess the same cost and delay as the best IGP ones going through $A2$), the two node segments can be replaced by a single one.

This correction is performed quickly and relies solely on information available to the router (the local SR graph and the received distances summary).
Finally, after having performed and corrected the cartesian products for all the ABRs of the area, the latter are merged in a single Pareto front.

% Finally, after having extracted the 3D Pareto fronts from the two ABRs, it is enough to return
%by updating the non-dominated paths according to this union of cartesian products.

Once performed for all areas, an ABR $A_x$ now possesses all 2COP paths to all considered destinations within the network. These can then be sent to routers within $\mathcal{A}_x$, who will need to perform similar computations to compute non-dominated paths to all routers within a different area.
Note that the 2COP paths for each destination can be sent as things progress, so that routers can process such paths progressively (and in parallel) if needed.\\

% Jro on peut peut êtr virer le summary si besoin
\textbf{Summary.} By running \bestcop within each area, before exchanging and combining the results, one can find all non-dominated paths to each destination within a network of \num{100000} nodes in less than 900ms. The induced message complexity is manageable in practice and can be further tuned if required. Our method can be
adapted for controller-oriented deployments.


% By knowing the SR graph of each zone, routers do theoretically
% know enough information to compute 2COP paths.








\subsection{A Limited Complexity with Strong Guarantees}
\label{sec:complexity}

\subsubsection{An Efficient Polynomial-Time Algorithm}
\label{sec:complexitybis}

\textbf{The flat \bestcop.} In the worst-case, for a given node $v$, there are up to $\mathit{degree}(v) \times \Gamma$
paths that can be extended towards it. Observe that $\mathit{degree}(v)$ is at least $|V|$ (because $G'$ is complete) and depends on how many parallel links $v$ has with its neighbors. With $L$ being the average number of links between two nodes in $G'$, \red{on average we thus have $\mathit{degree}(v) = |V|\times L \times \Gamma$ paths to extend to a given node, at worst.} These extensions are performed for each node $v$ and up to MSD times, leading to a complexity of $$O(c_0\cdot\Gamma\cdot |V|^2 \cdot L)$$
Using up to $|V|$ threads, one can greatly decrease the associated computation time.\\

%cpe: it is not the complexity that is decreased. Ißt is the overall computation time.
%reach a complexity of $O(c_0 \times |V| \times L \times \Gamma)$.
% In the worst-case \extendableIndex is of size $|V|$, and for each node, we iterate over all the edges of its successor. Hence those three ``for'' loops, in the worst case, iterate over all the edges in $E'$.
% For the fourth ``for'' loop, the size of \vardlist (the number of extendable paths for a given node) is at most $\Gamma$, by design. Procedure ExtendPaths is called at most MSD times, hence the given complexity.
% The complexity can then be rewritten as $O(MSD \times |V|^2 \times L \times \Gamma)$.

\textbf{The Cartesian Product.} Its complexity is simply the size of the 2COP solution space squared, for each destination, thus at worst $O((c_0 \cdot \Gamma)^2 \cdot |V|)$. Note that we can reach a complexity of $O(c_0^2 \cdot \Gamma^2)$, again with the use of $|V|$ threads since each product is independent. This worst case is not expected in practice as metrics are usually mostly aligned to result in Pareto fronts whose maximal size is much smaller than $c_0 \cdot \Gamma$.\\ %Moreover, if $o$ becomes too high, one can decrease the product $c_1 \cdot t$ to decrease $\Gamma$. %QB: je tente d'enlever ça, on verra si ça choque quelqu'un.

\textbf{Overall, \texttt{BEST2COPE} (multi-area) exhibits a complexity of}
\[
  O\left(c_0 \cdot \Gamma \cdot \left( c_0 \cdot\Gamma + L\cdot max_{\forall i \in [1..m]}(|V_i|) \right)\right)
  \]
  with $V_i$ denoting the set of nodes in each area $i$ ($m$ being their number) and the use of $|V|$ threads and sufficient CPU resources (\red{this bound is achievable ideally because the load is perfectly balanced and bottlenecks negligible}). Note that the cartesian product dominates this worst-case analysis as long as the product $V_i \cdot L $ remains small enough. However, with realistic weighted networks, we argue that the contribution of the Cartesian product is negligible in practice, so \texttt{BEST2COPE} is very scalable for real networking cases.
%\mathdisplay



\subsubsection{What are the Guarantees one can expect when the Trueness exceeds the Accuracy, \ie if $t > \gamma$ ?}
\label{sec:b2coplimits}
~\newline
\indent If propagation delays are measured with a really high trueness (\eg with a delay grain of 1 $\mu$s or less), \bestcop (and so, BEST2COPE) can either remain exact but slower, or, on the contrary, rapidly produce approximated results.
In practice, if one prefers to favor performance by choosing a fixed discretization of the propagation delay (to keep the computing time reasonable rather than returning truly exact solutions), this may result in an array not accurate enough to store all non dominated delay values, \ie two solutions might end up in the same cell of such an array even though they are truly distinguishable. Nevertheless, we can still bound the margin errors, relatively or in absolute, regarding constraints or the optimization objective of the 2COP variant one aims to solve.

%When true delays are more accurate than what \bestcop can afford, that is if the product delay accuracy ($t$) times delay constraint ($c_1$) requires more than $\Gamma =$ 1000 values % $c_1 . t > \Gamma = 1000$
%to store the whole Pareto front, \bestcop is no longer exact\footnote{As we will show in the next section, for large graphs having thousands of nodes, setting $\Gamma$ to $1000$ looks to be the limit to remain exact. However, \bestcop can rely on multiple threads to deal with higher $\Gamma$ efficiently.}. However, it still comes with strong guarantees thanks to the delay discretization. Such guarantees take the form of relative or absolute margin errors regarding constraints or optimization objectives depending on the 2COP variant one aims to solve.
In theory, note that while no exact solutions remain tractable if the trueness of measured delays is arbitrarily high (for worst-case DCLC instances), it is possible to set these error margins to extremely small values with enough CPU power. If $t < \gamma$, each iteration of our algorithm introduces an absolute error of at most $\frac{1}{\gamma}$ for the $M_1$ metric, \ie the size of one cell in our array (recall that $\gamma = \frac{\Gamma}{c_1}$ is the accuracy level and is the inverse of the delay grain of the static array used by \bestcop{}). So our algorithm may miss an optimal constrained solution $p^*_d$ (for a destination $d$) only if there exists another solution $p_d$ such that $d_1(p_d) \geq d_1(p^*_d)$ but the $M_1$ distance of both solutions associated to the same integer (that is stored in the same cell of the \vardist array) \ie only if $d_1(p_d) \leq d_1(p^*_d) + \frac{c_0}{\gamma}$. In this case, we have $d_2(p_d) \leq d_2(p^*_d)$ because otherwise, $p^*_d$ would have been stored instead of $p_d$.
From this observation, depending on the minimized metric, \bestcop{} ensures the following guarantees.

If one aims to minimize $M_0$ or $M_2$ (\eg when solving DCLC), then \bestcop guarantees a solution $p_d$ that optimizes the given metric, but this solution might not satisfy the given delay constraint $c \leq c_1$. As an example, for DCLC-SR (optimizing $M_2$), we have


$$d_0(p_d) \leq c_0$$
$$d_1(p_d) < c + \frac{c_0}{\gamma}$$
$$d_2(p_d) \leq d_2(p^*_d)$$
With $p^*_d$ denoting the optimal constrained solution.
When minimizing $M_1$, the solution returned by \bestcop for a given destination $d$, $p_d$, will indeed verify the constraints on $M_0$ and $M_2$, and we have $d_1(p_d) < d_1(p^*_d) + \frac{c_0}{\gamma}$.
The induced absolute error of $c_0/\gamma$ regarding the delay of paths becomes negligible as the delay constraint increases.
If $c \approx c_1$, the latter translates to a small relative error of $c_0/\Gamma$. Conversely,
it becomes significant if $c << c_1$. When minimizing $M_0$ or $M_2$, it is thus recommended to set $c_1$ as low as possible regarding the relevant sub-constraint(s) $c \leq c_1$ if necessary. Similarly, to guarantee a limited relative error when minimizing $M_1$, it is worth running our algorithm with a small $c_1$ as we can have $d_1(p^*_d) << c_1$.
However, note that this later and specific objective (in practice less interesting than DCLC in particular) requires some a priori knowledge, either considering the best delay path without any $c_2$ and $c_0$ constraints, or running twice \bestcop to get $d_1(p_d)$ as a first approximation to avoid set up $c_1$ blindly initially (here $c_1$ is not a real constraint, only $c_2$ and $c_0$ apply as bounds of the problem, $c_1$ just represents the absolute size of our array and, as such, the accuracy one can achieve).
% otherwise.

% Hence we have an absolute error of $c_0/\gamma$ regarding the constraint $c$. Note that this translate to a fairly small relative error of $c_0/\Gamma$ if $c = c_1$.
%Hence we have a relative error of $c_0/\Gamma$ for the $M_1$ metric
%(that can be divided by a factor 2 considering rounded values and constraints represented as integers as in our implementation).

%  Here the relative error may become significant if $d_1(p^*_d) << c_1$, \ie if the optimal constrained $M_1$ distance is much smaller than the maximal constraint $c_1$.
% In this case it is worth running our algorithm with a smaller maximal $c_1$, without changing $\Gamma$, to increase the accuracy $t$ and so guarantee a smaller relative error.


Even though \bestcop exhibits strong and tunable guarantees, it may not return exact solutions once two paths end up in the same delay cell, which may happen even with simple instances exhibiting a limited Pareto front.
%This flaw can be easily corrected through
Fortunately, a slight tweak in the implementation is sufficient to ensure exact solutions for such instances.
Keeping the original accuracy of M$_1$ distances, one can rely on truncated delays only to find the cell of each distance.
Then, one possible option consists of storing up to $k$ distinct distances in each cell\footnote{In practice, note that several implementation variants are possible whose one consists of using the array only when the stored Pareto front exceeds a certain threshold. Moreover, $k$ can be set up at a global scale shared for all cells or even all destinations, instead of a static value per cell, to support heterogeneous cases more dynamically. These approaches were also evoked in ~\cite{HIPH}}.
Thus, some cells would form a miniature, undiscretized Pareto front of size $k$ when required.
This trivial modification allows the complexity to remain bounded and predictable: as long as there exists less than $k$ distances within a cell, the returned solution is exact.
Otherwise, the algorithm still enforces the aforementioned guarantees.
While this modification increases the number of paths we have to extend to $k\cdot \Gamma$ at worst, such cases are very unlikely to occur in average. Notably, our experiments show that 3D Pareto fronts for each destination contain usually less than $\approx 10$ elements at most on realistic topologies, meaning that a small $k$ would be sufficient in practice.
In summary, \bestcop is efficient and exact to deal with simple instances and/or when $t \geq \gamma$, while it provides approximated but bounded solutions for difficult instances if $t < \gamma$ to remain efficient and so scalable even with massive scale IP networks.

\iffalse

In the basic DCLC-SR problem (\ie $2COP(s, c_0, c_1, \infty, M_2)$), and for each destination $d$, \bestcop returns a solution $sp'_d$ that verifies at worst: $d_1(sp'_d) < c_1 \cdot (1+\mathit{MSD}/\Gamma)$, $d_2(sp'_d) < c_2$ and $d_0(sp'_d) < c_0$. And if there exists an exact solution to the problem, say $sp_d$, then $d_2(sp'_d) \leq d_2(sp_d)$.

% <= opti segment

For other variants, like DCCLS (Delay-Cost Constrained with the Lowest \#Segment, \ie $2COP(s, 10, c_1, c_2, M_0)$), the guarantee turns out to be similar.
% because a constraint also applies on the delay
% , and since \bestcop looks for the minimal IGP cost it becomes also possible to virtually applies a constraint on it (a posteriori to check for the path existence).
The discretized delay is also constrained, leading to identical guarantees on the latter. Since \bestcop prefers paths of lower IGP cost, the paths found are bound to respect any feasible constraint on the IGP cost. We have $d_0(sp'_d) = d_0(sp_d)$ as the whole $M_0$ dimension is visited, regardless of the delay accuracy.
% = opti segments

% On a pas precisé Segment budget dans le premier cas alors ça me parait étrange de le préciser ici.
The CCLD-SR variant (Constrained Cost Lowest Delay in a SR context, \ie $2COP(s, c_0, c_1, \infty, M_1)$) is different, as the discretized value is here optimized. The guarantee is thus absolute for the $M_1$ metric (propagation delay). Formally, for each destination $d$, \bestcop returns $sp'_d$ that verifies at worst: $d_1(sp'_d) < d_1(sp_d) + \mathit{MSD}/t$, $d_2(sp'_d) < c_2$ and $d_0(sp'_d) < c_0$, where $sp_d$ is an optimal solution.


% However for the CCLD-SR variant (Constrained Cost Lowest Delay in a SR context -- with a \#Segment budget), while we still have a guarantee it is, by definition, not longer relative to the delay constraint but absolute and only regarding the delay optimization objective. Basically, it entirely depends on the delay grain. Formally, we have: for each destination $d$, \bestcop return solution $sp'_d$ that verifies at worst: $d_1(sp'_d) - d_1(sp_d) < 1/t$, $d_2(sp'_d) \leq d_2(sp_d) < c_2$ and $d_0(sp'_d) =  d_0(sp_d) < MSD$.

Finally, recall that when exact, solving 2COP allows to solve
stricter sub-problems, \ie we consider large constraints to also solve instances with tighter constraints: $c'_k << c_k$. However, when the delay accuracy becomes too high to store the whole Pareto front, 2COP maintains a subset of the front. More precisely, solving 2COP for $c_1 = 100$ and $\Gamma = 1000$ leads to a error margin of 0.01ms (0.1\% relative to $c_1$). However, if one wants to retrieve a stricter subproblem solution, \eg $c_1 = 1ms$ (if the accuracy allows such small constraints to carry any meaning), the error of 0.01ms becomes of 10\% relative to the constraint. In other words, in such cases, it becomes more reasonable to re-run \bestcop for a smaller constraint and adapt
the delay grain (for example a grain of $c_1/1000 = 1\mu$s for a constraint of 1ms comes with an error margin of at worst 0.5\%).
% $t$ to $c_1$, setting $t = \frac{\Gamma}{c_1} = 1000/c_1$ and the delay grain to $c_1/1000$, that is for example a grain of 1$\mu$s for a constraint of 1ms. This allows to ensure a relative margin error of at worst 0.5\% for all segment list / path ($MSD/2t = 10/2000 = 0.005$) regarding the $c_1$ constraint in any cases. In other words, the returned path (if one exists) cannot exceed the constraint more than what \bestcop guarantees, e.g., a worst margin of 5$\mu$s for a constraint of 1ms.

% note that when the delay accuracy is too high to store the whole Pareto front, 2COP is no longer as suitable as in the exact case in its extension mode (that ); it becomes more reasonable to adapt $t$ to $c_1$ and so setting $t = \frac{\Gamma}{c_1} = 1000/c_1$ and the delay grain to $c_1/1000$, that is for example a grain of 1$\mu$s for a constraint of 1ms. This allows to ensure a relative margin error of at worst 0.5\% for all segment list / path ($MSD/2t = 10/2000 = 0.005$) regarding the $c_1$ constraint in any cases. In other words, the returned path (if one exists) cannot exceed the constraint more than what \bestcop guarantees, e.g., a worst margin of 5$\mu$s for a constraint of 1ms.

% The last variable is the most sensitive as, although like others it has only a linear impact on the complexity, it can grow fast according to the necessary/expected accuracy of one-way propagation delay measurements.
% In fact, if $\Gamma$ is very high due to extra-fine grain accuracy of measurements (e.g., sub-microsecond trueness), \vardist[\varn] can be converted to a hashmap instead of an array. Indeed, doing so, the memory usage of \vardist[\varn] would not depend on $\Gamma$ but rather on the size of the Pareto front (that we expect to be lower than the $M_2$ theoretical spreading thanks to a limited amount of distinct distances), at the cost of a slightly slower insertion, and memory access, which will depend on the number of distinct distances (but not directly on the spreading).

\fi


==> clean_latex/sections/bio.tex <==
% !TEX root = ./paper.tex
\vspace{-1cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {JRL.pdf}}]{Jean-Romain Luttringer} received his master's degree in
  Computer Science from the University of Strasbourg (France) in 2019, where
  he is currently a Ph.D. candidate within
  the Networks Research Group of the ICube laboratory. His research interests
  includes routing and path computation.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {alfroy.jpeg}}]{Thomas Alfroy} received his master's degree in Computer Science from the University of Strasbourg (France) in 2021. He is currently a Ph.D student within the Network Research Group of the ICube laboratory. His research topics are Network anomaly detection and BGP.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {Quentin.pdf}}]{Quentin Bramas}  received a M.Sc. in Computer Science from
  Nancy University (France, 1972), a Ph.D. in Computer Science from Cornell
  University (USA, 1976).
  % and a ``Doctorat d'Etat'' from the University of Strasbourg (France, 1983).
  He joined the Department of Computer Science from the same University where he was successively appointed as Assistant Professor, Associate Professor, and Full Professor (1984). He led the Network and Protocol group of the LSIIT Laboratory and is now retired. His research interests included
  % routing, multicasting,
  traffic engineering and Internet cartography.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {Pascal.pdf}}]{Pascal M\'erindol} received his Ph.D. degree from the
  University of Strasbourg (France) in 2008. Then, he spent two years in Belgium
  at the Universit\'e catholique de Louvain as a post-doctoral researcher. He is now
  Associate Professor at the Networks Research Group of the ICube laboratory in the University of Strasbourg. His main research topics are routing and Internet measurements.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {Cristel.JPG}}]{Cristel Pelsser} received the Ph.D. degree from the Université catholique de Louvain (UCLouvain), Belgium. She has spent nine years working for ISPs. She has been a Professor with the University of Strasbourg since November 2015. She leads a team of researchers focusing on core Internet technologies. Her aim is to facilitate network operations, and to avoid network disruptions.
\end{IEEEbiography}


==> clean_latex/sections/conclusion.tex <==
\section{Conclusion}
While the overhead of MPLS-based solutions lead to a TE winter in the
past decade, Segment Routing marked its rebirth. In particular, SR enables the
deployment of a practical solution to the well-known DCLC problem. \red{Our algorithm,
\bestcop~\cite{nca2020} (Best Exact Segment Track for 2-Constrained Optimal Paths), iterates on the SR Graph to natively solve DCLC in SR domains with strong guarantees, through simple and efficient data structures and concepts.}
% ; either with exactitude for simple instances (\ie with Pareto fronts limited in size and/or weak delay trueness) or, at worst for difficult instances, with strong guarantees, \eg a bounded distance regarding the delay constraint.

% Indeed, \bestcop not only handle SR as a third constraint almost for free, but also relies on the most simple and efficient data structures and concepts available in the DCLC literature.

In this paper, we went several steps further with the following achievements:
\begin{itemize}
\item experimentally demonstrating that SR is a relevant technology to deploy DCLC paths;
% , the vast majority of solutions are not exceeding its MSD limit (\ie the required number of segments is limited to 10 in practice);
% \item the versatile design of \bestcop allows ISP to solve the most practical category of optimization variants and heterogeneous constraints for each destination within SR domains, \ie it solves 2COP taking into account the propagation delay, the IGP cost and the number of necessary segments;
\item for massive scale ISPs relying on area-subdivision, we extend \bestcop to \bestcope, partitioning 2COP into smaller sub-problems, to further reduce its overall complexity (time, memory and churn);
\item through extensive evaluations, relying on multi-threading and our own multi-metric/multi-areas network generator, we have shown that \bestcope is very efficient in practice. This was confirmed through a comparison with a relevant state-of-the-art algorithm, which benefited from a novel path to segment multi-metric conversion algorithm that we designed.
\end{itemize}

To the best of our knowledge, \bestcop is the first practically exact and efficient solution for 2COP within SR domains, making it the most practical candidate to be deployed for such a TE flavor in today ISPs.
It is able to solve 2COP on massive scale realistic networks having \num{100000} nodes in less than a second.
For large areas having thousands of routing devices, we have shown that \var{BEST2COP(-E)} can easily deal with random topologies while its competitors do not scale.
Finally, more advanced and flexible structures can be envisioned to deal with high trueness requirements, while deploying novel flex-algo strategies can help to mitigate the rare SR limit drawbacks.


\section*{Acknowledgment}
This work was partially supported by the French National Research Agency (ANR) project Nano-Net under contract ANR-18-CE25-0003.

==> clean_latex/sections/evaluation.tex <==

\section{Performance Evaluation}
\label{sec:evaluation}
% I don't know if I should say that we consider that we're exact,
% to prevent the "Samcra is exact and you aren't" debate
% I ended up writing it but feel free to remove it.

In this section, we evaluate the computation time of our solution.
We start by evaluating \bestcop on various flat network instances, ranging from worst-case scenario to real topologies, and compare it to another existing approach based on the \textit{Dijkstra} algorithm, \samcra~\cite{SAMCRA}.
Then, after having introduced our multi-area topology generator, we evaluate the extended variant of our solution, \bestcope, on massive scale networks.
In the following, we consider our discretization to be exact (\ie $\Gamma$ is high enough to prevent loss of relevant information).


\red{To conduct our evaluations, we consider that:}
\begin{itemize}
 \item $c_0 = \mathit{MSD} = 10$, as it is close to the best hardware limit;
 % but, in most of the cases, we will show that, for realistic topologies, the number of necessary iterations is lower than this limit (BEST2COP stops naturally before with the optimal solutions since there is no progress in the algorithm, no more paths can be extended);

\item $L = 2$: \red{while some pairs of nodes may have more than two parallel links connecting them in $G$, we argue that, on average in $G'$, one can expect that the total number of links in $E'$ is lower than $2|V|^2$.}
%  Indeed, while one node and several adjacency segments can co-exist for a given pair $(u,v)$ in $E'$, adjacency segments are not likely to be numerous within transformed graphs (they tend to either be dominated by the node segment or dominated by another adjacency one);

 % should not be dominated between themselves and regarding the node segment for this to occur;
 \item $\Gamma = 1000$, although this value is tunable to reflect the expected product trueness-constraint on $M_1$, we consider here a fixed delay grain of 0.1ms (so an accuracy level of $\gamma = 10$) regarding a maximal constraint $c_1 =$ 100ms. This $\Gamma$ limitation is realistic in practice and guarantees the efficiency of \bestcop even for large complex networks as it becomes negligible considering large $|V|$.

\end{itemize}

\red{Note that the delays fed to \samcra are \emph{also} discretized in the same fashion as for \bestcop, allowing the number of non-dominated paths that \samcra has to consider to be bounded and reduced.}
\red{In addition, as \samcra is not designed with the SR Graph in mind, it is difficult to know which of the two methods mentioned in Section~\ref{ssec:srgraph} is the most suited to consider the segment metric. Thus, we compare ourselves to both variants. First, we run \samcra on the fully-meshed SR Graph, which allows to use the \samcra algorithm nearly as-is. We call this variant \samcrasrg. Second, we implement our conversion algorithm, which allows to efficiently convert multi-metric paths to segment lists. This method requires however further modification of the \samcra algorithm, not only by adding the conversion algorithm but also by extending its dominancy checks (details can be found in Appendix~\ref{app:LCA}). We refer to this variant as \samcralca.\\}
    



%(\ie not a 3D Pareto Front, but a 2D Pareto front where not path exceeds MSD edges). 
All our experiments are performed on an Intel(R) Core(TM) i7-9700K CPU @ 3.60GHz $\times$ 8.

\subsection{Computing Time \& Comparisons for Flat Networks}
This section illustrates the performance of our algorithm \bestcop using three flat network scenarios.
In particular, we do not take advantage of any area decomposition to mitigate the computing time.

\red{As shown in \cite{nca2020} by forcing \bestcop to explore its full iteration space, our algorithm \emph{cannot} exceed 80s at worst on topologies of \num{1000} nodes. This upper bound can however be drastically reduced through the use of multi-threading, reaching a worst-case of $\approx 10s$ when relying on 8 threads, highlighting the parallel nature of our algorithm~\footnote{Additional experiments on a high-performance grid showed that \bestcop may reach a speed-up of 23 when running on 30 cores.}. Additional information can be found in Appendix~\ref{upper_bound} for the interested reader. }

\red{We will see that in practice, \bestcop is far from reaching these upper bounds, even on random networks. In the following, we will evaluate \bestcop and compare it to \samcra in two main scenarios: a real network with real link valuations, and random networks of up to \num{10000} nodes.\\}



\begin{figure*}[!ht]
    \centering
    \caption{Computation time of \bestcop and \samcra on various experiments. Although the results can be close when considering mono-threaded \bestcop and \samcra, our algorithm always outperforms its competitor when using multi-threading. In some cases, multi-threading is not even necessary}\label{fig:allEvals}
        \subfloat[Computation time of \bestcop (1, 2, 8 threads) \& \samcra on a real network with real link valuation.]{\includegraphics[width=0.32\linewidth]{geo-Violin.pdf}}\label{fig:geoSprint}
        \hspace{0.1em}
        \subfloat[Computation time of \bestcop \& \samcra on random networks with random valuation for $|V| = 100$ to \num{1000}]{\includegraphics[width=0.32\linewidth]{1K.pdf}}\label{fig:1K}
        \hspace{0.1em}
        \subfloat[Computation time of \bestcop \& \samcra on random networks with random valuation for $|V| =$ \num{1000} to \num{10000}]{\includegraphics[width=0.32\linewidth]{10K.pdf}}\label{fig:10K}
\end{figure*}

\textbf{Real network.}
%Our basic settings are left unchanged, \ie $\Gamma = 1000$ and \bestcop still does not take advantage of any distance pruning to reduce $G'$.
\red{We start by considering a real IP network topology. We use our largest available ISP topology, consisting of more than 1100 nodes and 4000 edges. \red{This topology describes the network of a Tier-1 operator and is not available to the public}~\footnote{While public topology datasets exist, these topologies are often too small for our use-case and/or do not possess any link valuation.}.
While the IGP costs of each link were available, we do not have their respective delays.
We thus infer delays thanks to the available geographical locations we do possess: we set the propagation delays as the orthodromic distances between the connected nodes divided by the speed of light, and run both algorithms on the obtained topology. The execution times are then shown in Fig.~\ref{fig:geoSprint}. \bestcop (1, 2, 8 threads) and \samcra (with LCA and SRG) are run for every node as source, resulting in the distributions showcased.}


\red{One can see that \samcrasrg (\ie \samcra run directly on the SR Graph) exhibits the worst execution times out of all the algorithms and variants presented, averaging at $100$ms, and reaching $250$ms at worst.
Interestingly, this shows that exploring the SR Graph itself may be detrimental to some algorithms (in particular priority-queue-based ones) due to its high density. Hence, algorithms not designed to take advantage of its features may fare better by exploring the original, sparser topology, and using the information within the SR Graph to compute the number of necessary segments to encode the paths being explored. This is visible on \samcralca computation times. Our construct, coupled with our conversion algorithm, allowed \samcralca to reach computation times very similar to the mono-threaded variant of \bestcop, with an average execution time of $\approx 60$ms. Note that \bestcop, which runs on the SR Graph itself, shows equivalent execution time when relying on a single thread. However, when relying on multiple threads, \bestcop outperforms its competitor in all runs, reaching a computation time of $\approx 25$ms at worst when using 8 threads, \ie three times faster than its competitor.}




% One can see that the two algorithms indeed benefit from interesting properties in deployed networks.
% In particular, the execution time of \bestcop rarely exceeds 25ms (resp. 100ms)
% when relying on 8 (resp. 1) thread.
% Performance are greatly enhanced compared to previous cases thanks to the
% real underlying network structure and weights alignement: few distances dominate all the others leading to small Pareto front.  %because metrics are often aligned in practice.
% A similar trend can be observed for \samcra, whose average execution time decreases drastically compared to the previous evaluation, to reach $\approx 130$ms, although some outliers took $350$ms.
% These results are not surprising, as \samcra, as well as other Dijkstra-like related approaches, rely on the fact that simple practical cases result in small Pareto fronts, as metrics are often somewhat aligned.
% cpe: how does performance degrade as the percentage of unaligned weights increases?
% Note JRO: TODO future work, c'est pas évident à mesurer

% probably due to the density of the SR graph,
% Nevertheless, \bestcop still shows better performance (be it with a single or multiple threads), in particular because of the density of the SR graph input that impacts both approaches. Indeed, \samcra, being implemented with a binary heap as priority queue, is more likely to suffer from large $|E|$ than \bestcop.

These low execution times are not only due to the efficiency of the algorithms presented, but also to the realistic link valuations, which tend to be correlated in practice. In realistic cases, \bestcop can thus work with $\Gamma > 1000$ and so with a supported accuracy $t >> 0.1$ms (to deal with a micro-second grain) for small enough delay constraint (\ie, $<< 100$ms), while keeping the execution time in the hundreds of milliseconds.
One may notice that (almost) perfectly aligned metrics reduce the usefulness of any DCLC-like algorithm, but such metrics are not always aligned for all couples in practice (even with realistic cases, we observe that the average size of the 3D Pareto front is strictly greater than $1$, typically $\approx 4$). Our algorithm deals efficiently with easy cases and remains exact\footnote{Or at least near exact for difficult instances having both high trueness and exponential increasing Pareto fronts.} and efficient for more complex cases, \eg with random graphs.\\








% The networks used so far were flat networks, with sizes typically not exceeding a thousand nodes.
% However, some recent IP network deployments exceed \num{10000} nodes even in medium-sized countries. We thus now aim to evaluate the execution time of \bestcope, the extended variant of \bestcop which supports and leverages OSPF-like area division. This version is adapted to tackle TE problems in massive scale, hierarchical networks.\\

% In the following, we only consider our approach, as it already exhibited better performance than \samcra even for small simple instances. However, before continuing analyzing the computing time results, we first introduce our generator for massive-scale, multi-areas, realistic networks having two valuations.


\red{\textbf{Random networks. } The number of publicly available large topologies being limited, we continue our evaluation with random scenarios to assess the computation time of the aforementioned algorithms on a larger number of scenarios.}


\red{We generate raw connected graphs of $|V|$ nodes by using the Erdos-Rényi model. The generated topologies have a degree of $log(|V|)$. Both the delays and the 
IGP weights are picked uniformly at random. IGP weights are chosen within the interval $[1, 2^{32} / |V| / 10]$, to ensure that no paths possesses a cost higher than $2^{32}$. Delays are chosen within the interval $[0, 0.01 \times c_1]$, with $c_1 = 100ms$, to ensure that a high number of feasible paths exist.}

\red{We start by running \bestcop and \samcra for $|V|$ ranging from 100 to 1000 (with steps of 100). To account for the randomness of both valuation functions, we generate 30 differently weighted distinct topologies for each value of $|V|$. We run \bestcop and \samcra for 30 nodes selected as representative sources (randomly picked uniformly). Computing times are shown in Fig~\ref{fig:1K}.}


% The number of threads is set to $T = 1$ and $8$ as shown in Fig~\ref{fig:RND}. While \samcra is run from the same amount of sources in the same conditions, it cannot benefit as-is from multi-threaded architectures, as it cannot be parallelized as easily. Note that \samcra is also run on the SR Graph, to spare it the management of a 3D Pareto front (\ie on the fly conversions into segment lists of the discovered paths to perform continuous Pareto front updates).

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.55]{10K.pdf}
%     \caption{Computation time taken by \bestcop (1,4 and 8 threads) and \samcralca to solve 2COP on random topologies with random weights. Weights are uniformly distributed between 0 and 1\% of the constraint. Each topology has an average degree of $log(|V|)$.}
%     \label{fig:RND}
% \end{figure}

% Note that such an evaluation is not advantageous and not yet representative of the times reached on real instances. We do not benefit from the patterns present in realistic networks such as metric alignment.
% Such random valuations exhibit the efficiency of \bestcop in moderate challenging conditions.
% When relying on a single thread, \bestcop reaches an execution time of
% about $250$ms when $|V| = \num{1000}$. Once again, this time can be greatly reduced when relying on multiple threads. With 8 threads, \bestcop remains under 100ms in all of its runs (below this \#node threshold),
% exhibiting an average performance of about 50ms when $|V| = \num{1000}$.
% Overall, \bestcop scales well enough with the dimension of the network which is the critical performance parameter (quadratic in $|V|$). 

% \samcra showcases a higher execution time, reaching $250$ms for $|V| = \num{400}$, and 2s when $|V| = \num{1000}$. The latter suffers far more from the density of the SR graph (to natively manage the third dimension of the Pareto front), and mostly from the random nature of the weights that impacts the size of the Pareto front. Indeed, while \bestcop perform updates of the Pareto front in a relaxed amortized manner at the end of each iteration, \samcra updates it for each new discovered path resulting in a higher management cost when the front size becomes significant.


\red{While the computation times are slightly higher (due to the random valuations which lead to a higher number of non-dominated paths), the results are similar to the previous experiment. These results display more clearly that \samcra does not benefit from exploring the SR Graph. Indeed, on random networks, \samcrasrg is about 7 times slower than the other algorithms displayed. 
However, as on real networks, \samcralca shows results close (if not equal) to \bestcop execution time. Nevertheless, even on random networks, \bestcop remains three times faster than its competitor when relying on 8 threads.}

\red{Interestingly, \bestcop mono-threaded and \samcralca computation times get closer as $|V|$ increases. Thus, we continue our comparison on networks of \num{2000} to \num{10000} nodes. Given the long computation times of \samcrasrg, we here only consider \samcralca. The results are shown in Fig.~\ref{fig:10K}.
On such networks, \bestcop (mono-threaded) exhibits an execution time of $7s$, while \samcralca remains under $5s$. The quadratic complexity of \bestcop (whose main factor is $|V|^2$) is here clearly visible. 
\samcralca exhibits a less steep growth. However, when relying on multiple-thread, \bestcop remains far more efficient. While two threads already allow to reach an execution time slightly lower than \samcra (4s), 8 threads allow \bestcop to remain $\approx 3.3$ times faster than its competitor.} \\

\red{\textbf{Summary.} The way to use the SR Graph has a high impact on the underlying algorithm. As the SR Graph is not at the core of 
\samcra's design, exploring the latter lead to high execution time due to its density. However, adding our conversion algorithm (which relies on the SR Graph data) within \samcra allowed the latter to reach competitive execution times while solving 2COP. \bestcop, which explores the SR Graph directly, exhibits an execution similar to \samcralca when relying on a single thread. When using multi-threading, \bestcop clearly outperforms its competitor in all scenarios.\\}

In any case, it is interesting to note that even \bestcop takes more than one second on networks of \num{10000} nodes. To showcase the performance of our contribution on massive-scale networks, we now evaluate the execution time of its extension, \bestcope, which supports and leverages OSPF-like area division. This version is adapted to tackle TE problems in massive-scale hierarchical networks. In the following, we only consider our approach. Indeed, the latter showcased better performance that \samcra even without relying on multiple threads when considering a topology size $|V| < 1000$, which encompasses the size of standard OSPF areas.

However, before continuing analyzing the computing time results, we first introduce our generator for massive-scale, multi-areas, realistic network having two valuations (IGP cost \& delays).


% TODO CHECK TOPOLOGY ZOO

% \begin{figure}
%     \includegraphics[scale=0.5]{geo-Violin.pdf}
%     \caption{\red{Computation time taken by \bestcop (1 and 8 threads) and \samcra (SRG \& LCA) to solve 2COP on a real topology with real weights ($|V| \approx \num{1000}$)}.}
%     \label{fig:RLT}
% \end{figure}



\subsection{Massive Scale Topology Generation}
\label{sec:generator}

% \subsection{Generating Realistic Large Graphs}
To the best of our knowledge, \red{although such networks exist in the wild,} there are no massive scale topologies
made \red{\textit{publicly}} available which exhibit IGP costs, delays, and area subdivision.
For example, the graphs available in the topology zoo (or sndlib) datasets do not exceed 700 nodes in general. Moreover, the ones for which the two metrics can be extracted, or at least inferred, are limited to less than 100 nodes.
Thus, at first glance, performing a practical massive-scale performance evaluation of \bestcope is highly challenging if not impossible.
There exist a few topology generators~\cite{IGEN, BRITE} able to generate networks of arbitrary size with realistic networking patterns, but specific requirements must be met to generate topologies onto which \bestcope can be evaluated, in particular the need for two metrics and the area decomposition.\\

\textbf{Topology generation requirements. }
First, the experimental topologies must be large, typically between \num{10000} and \num{100000} nodes.
Second, they must possess two valuation functions as realistic as possible, one for the IGP cost and the other modeling the delay.
Third, since the specific patterns exhibited by real networks impact the complexity of TE-related problems, the generated topologies must possess realistic structures (\eg with respect to redundancy in the face of failures in particular).
Finally, for our purposes, the topology must be composed of different areas centered around a core backbone, typically with two ABRs between each to avoid single points of failure. % (following standard OSPF architecture s).
%To the best of our knowledge, current topology generators fail to address all of these requirements.
Since we do not know any generator addressing such requirements, we developed YARGG (Yet Another Realistic Graph Generator), a python tool(Code available online~\footnote{\url{https://github.com/JroLuttringer/YARGG}}) which allows one to evaluate its algorithm on massive-scale realistic IP networks. In the following, we describe the generation methods used to enforce the required characteristics.\\

\textbf{High-level structure.}
One of the popular ISP structure is the three-layers architecture~\cite{CampusNe63:online}, illustrated in Fig.~\ref{fig:area}. The \textit{access layer} provides end-users access to the communication service. Traffic is then aggregated in the \textit{aggregation layer}. Aggregation routers are connected to the
\textit{core routers} forming the last layer. The aggregation and access layers form an area, and
usually cover a specific geographical location. The core routers, the ABRs connecting the backbone other areas, and their links, form the backbone area that interconnect the stub areas, \ie the aggregation and access layers of the different geographical locations. Core routers are ABRs and belong both to a sub-area, per couple of 2 for redundancy.
Thus, while the access and aggregation layers usually follow standard structures and weight systems recommended by different network vendors, the backbone can vastly differ among different operators, depending on geographical constraints, population distribution, and pre-existing infrastructure. Taking these factors into account, YARGG generates large networks by following this 3-layer model, given a specific geographical location (\eg a given country).\\

\begin{figure}
    \centering
    \includegraphics[scale=0.15]{triple_weight.png}
    \caption{Core network (before step 5) generated by YARGG in France. While we consider the road distances, we represent the links in an abstract fashion for readability purposes. The color and width of the links represent their bandwidth (and thus their IGP costs).}
    \label{fig:coreFR}
\end{figure}

\textbf{Generating the core network and the areas. }
YARGG is a heuristic that generates the core network by taking the aforementioned considerations into account: existing infrastructures, population, and geographical constraints.
An example of a core network as generated by YARGG may be
seen in Fig.~\ref{fig:coreFR}.
Given a geographical location (e.g., a country or a continent), YARGG builds the structure of the core network by
 \begin{enumerate}
    \itemsep0em 
     \item \emph{Extracting the $x$ most populated cities in the area}. Close cities are merged in a single entity.\red{ The merge trigger value may change (the exact values used here can be found in ~\cite{topologies})}.
     \item \emph{Constructing a minimum Spanning-Tree covering all cities of the area}, using road distances as the metric. \red{Links between cities totaling more 
     than 30\% of the total population are normalized in order to be highly prioritized.\footnote{The parameters tuned may be easily modifier. For now, the latter are purely empirical.}}
     \item \emph{Removing articulation-points.} \red{YARGG picks one bi-connected component, and adds the smallest link (in terms of road distances) that 
     bridges this component with another. This process is repeated until no articulation point remains (\ie the topology is bi-connected).}
     \item \emph{Adding links increasing the connectivity and resilience for a limited cost.} \red{YARGG considers all links meeting certain criterias. The two cities/nodes must be closer than 20\% of the largest road distance. Their current degree must be lower than 4. The link, if added, should reduce the distance (and so, the delay) between the nodes by at least 25\%. Among these links, YARGG adds the one with the highest attractiveness, expressed as the sum of the distance reduction and the population of the cities (normalized).}
     \item \emph{Doubling the obtained topology.} The topology is doubled. There are now two nodes (/routers) per city. Links are added between the two routers of the same city, making the topology tri-connected.
 \end{enumerate}


The couple of routers located at each city within this generated backbone area become the ABRs between the backbone and their area, which is generated next.\\

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{AREA.pdf}
    \caption{Weights and structures of an area generated by YARGG.}
    \label{fig:area}
\end{figure}

\textbf{Access \& aggregation layers. }
These last two layers make up a non-backbone area and span a reduced geographical area.
Thus, one access and one aggregation layer are located in each city considered by YARGG.
Several network equipment vendors recommend a hierarchical topology, such as the three-layer hierarchical model~\cite{Hierarch47:online}. An illustration can be seen in Fig.~\ref{fig:area}.
Simply put, there should be two core routers (the ABRs) at the given location (a city in YARGG's case).
Each core router is connected to all aggregation routers. For better resiliency, the aggregation layer is divided into aggregation groups, composed of two connected routers.
Finally, routers within an aggregation group are
connected to access-layer routers. To achieve areas of $\approx$ 300 nodes, we consider 30 access routers per aggregation group. This results in a large, dense, and realistic graph. \\

\textbf{Weights. } In the backbone, the weights generated by YARGG are straightforward.
The delays are extracted from the road distances between the cities, divided by $60\%$ the speed of light (close to the best performing fiber optic). The IGP cost is 1 for links between large cities since these links usually have a high bandwidth (in black in Fig.~\ref{fig:coreFR}), 2 for standard links, necessary to construct a tri-connected graph (added at step 3, in red in Fig.~\ref{fig:coreFR}), and 5 for links that are not mandatory, but that increase the overall connectivity (added at step 4, in orange in Fig.~\ref{fig:coreFR}).

Within an area, the IGP costs follow a set of realistic
constraints, according to two main principles:
(i) access routers should not be used to route traffic (except for the networks they serve), (ii) links between routers of the same hierarchical level (\eg between the two core routers or the two aggregation routers of a given aggregation group) should not be used, unless necessary (\eg multiple links or node failures). These simple principles lead to the
IGP costs exhibited in Fig.~\ref{fig:area}.
The delays are then chosen uniformly at random.
Since access routers and aggregation routers are close geographically, the delay of their links is chosen between $0.1$ and $0.3$ms. The delay between aggregation routers and core routers is chosen between $0.3$ms and the lowest backbone link delay.
Thus, links within an area necessarily possess a lesser delay than core links.\\


\textbf{Summary. } YARGG computes a large, realistic, and multi-area topology. The backbone spans a given geographical location and possesses simple IGP weights and realistic delays. Other areas follow a standard three-layer hierarchical model. Weights within a stub area are chosen according to a realistic set of usual ISP constraints. Delays, while chosen at random within such areas, remain consistent with what should be observed in practice.

\subsection{Computing Time for Massive Scale Multi-Areas Networks}
\begin{figure*}
    \centering
    \includegraphics[scale=0.45]{BEST2COPE_TNSM.pdf}
    \caption{\bestcope computation time on 5 continent-wide topologies generated by YARGG.}
    \label{fig:bcope}
\end{figure*}

Using YARGG, we generate five massive scale, continent-wide topologies, and run \bestcop on each one of them. The topologies ranges
from \num{10000} to \num{100000} nodes. 
% TODO maybe I need to extract some properties of the topologies ? cpe: yes, that may be useful.
% Note JRO: TODO
Each non-backbone area possess around \num{320} nodes. The topologies, their 
geographical representations and some of the associated network characteristics can be found online~\cite{topologies}.

We run \bestcop on each ABR as a source (around $|V| / 320 \times 2$ sources). The time corresponding to the message exchange of the computed Pareto front (step 2 of \bestcope) is not taken into consideration. Thus, 
% the experiment is comprised of the following steps:
% \begin{enumerate}
% \item All ABRs run \bestcop for their areas and convert the found distances into segment lists;
% \item The current source ABR performs the Cartesian product of distances as described in Sec.~\ref{sec:areas}, to find all non-dominated distances to all $|V|$ destinations.
% \end{enumerate}
the computation time showcased is the sum of the average time taken by ABRs to perform the preliminary intra-area \bestcop (and the distances to segment lists conversions) plus the time taken to perform the $|V| / 320 \times 2 - 2$ Cartesian products (for all other ABRs of all other areas).

Note that we consider an ABR as a source and not an intra-area destination.
In practice, the ABR would send the computed distances to the intra-area nodes, who in turn would have to perform a Cartesian product of these distances with its own distances to said ABR.
However, both the ABR and the intra-area node have to consider the same number of destinations ($|V|$), and the results computed by the ABR can be sent as they are generated (destination per destination), allowing both the ABR and the intra-area nodes to perform their Cartesian product at the same time. In addition, intra-area nodes may benefit from several optimizations regarding their Cartesian product, if the constraints of the desired paths are known (these optimizations will not be used nor detailed in this paper).
For these reasons, we argue that the time measured here, using an ABR as a source, is representative of the total actual time required, \ie the overall worst time for the last treated destination at each source.

The results of this experiment are shown in the violin plot of Fig.~\ref{fig:bcope}.
By leveraging the network structure, \bestcope exhibits very good performance despite the scale of the graph.
For \num{10000} nodes, \bestcope exhibits a time similar to the one taken by its flat variant for $|V| = 2000$.
Furthermore, \bestcope seems to scale linearly with the number of nodes, remaining always under one second for $|V| \approx \num{75000}$. Even once the network reaches a size of $\approx \num{100000}$, \bestcope is able to solve 2COP in less than one second for a non-negligible fraction of the sources, and never exceeds 1.5s.

Note that the times showcased here rely on a single thread.
While \bestcope's Cartesian product can be parallelized locally (both at the area and the destination scale), this parallelization hardly has any effect. This is explained by the fact that these individual computations are in fact fairly efficient, hence the overhead induced by the creation and management of threads is heavier than their workload. In addition, since \bestcop deals with very large topologies, some complex memory-related effects might be at play. Indeed, we notice these results to surprisingly vary depending on the underlying system, operating system, and architecture due to the differences in terms of memory management.

Thus, while massive scale deployments seem to a priori prevent the usage of fine-grained TE, their structures can be leveraged, making complex TE problems solvable in less than one second even for networks reaching $\num{100000}$ nodes. The computations performed for each 
area can also be distributed among different containers 
within the cloud, if handled by a controller.

% \subsection{Discussions and Ongoing Works}\label{sec:discussions}

% The absolute times exhibited here may surprise some readers.
% Well-known algorithms, such as MC Dijkstra (similar to \samcra, except for a different cost function), have been shown to solve DCLC exactly, in about 300ms in road networks of \num{250000} nodes~\cite{Hanusse_Ilcinkas_Lentz_2020}.
% In our evaluation, \samcra reaches this execution time for one thousand nodes only.

% However, such experiments only consider two dimensions (cost and delay), and do not consider Segment Routing (neither as a third dimension or with an SR graph).
% Consequently, these best time DCLC results are usually performed on very sparse networks (usually real or random ones, with a density that may be as low as 0.0001) with aligned metrics. In our study, algorithms are run on very dense SR graphs (density of 1 for each flat network or area), to natively consider the number of segments and fully solve 2COP (or at least DCLC-SR for \samcra in our comparisons).

% As one may recall, considering the fully meshed SR graph has two main advantages.
% First, it allows to easily consider the number of segments and the associated MSD constraint.
% Maintaining a 2D Pareto front is then sufficient, as the third dimension can be handled natively.
% Second, it prevents the need of converting all discovered paths to segment lists on the fly.
% Indeed, the number of segments characterizes a path, not an edge.
% In other words, this metric cannot be added to the weight vector of an edge. Rather, all discovered paths must be converted to segment lists to maintain a correct 3D Pareto front, respecting the MSD constraint.
% % If one ignores the number of segments when computing paths, the resulting Pareto front may turn out to be solely composed of unfeasible paths exceeding the MSD constraint.  Thus, this conversion is necessary. JRO: maybe uncomment this
% Although the information required to perform this conversion in polynomial time is available, it would require many additional computations.

% For these reasons, we considered here that running algorithms on the SR graph itself is beneficial.
% Indeed, \bestcop has the ability to handle path updates without the use of any PQ, such that it is less sensitive to this graph parameter than Dijkstra related approaches that may suffer from dense graphs, such as SR ones, if relying on a naive PQ implementation.
% While most algorithms maintain the Pareto front up to date as soon as a path is visited, \bestcop only perform this operation once per iteration. Thus, the maintenance cost is lower and less dependent on the number of edges.
% For Dijkstra based approaches such as \samcra, the use of a relaxed PQ (like the Fibonnacci heap) may look useful to decrease this sensitivity.
% However, in our evaluations, we consider a binary heap to implement the PQ of \samcra as it is the one providing the best performance in the scope of our experiments. Indeed, just marking a path as deprecated in the binary heap is enough to relax the updates (\ie there is no need to re-organize the heap at a logarithmic cost).

% Moreover, it is thus worth investigating if using the SR graph is actually detrimental to other algorithms, including \samcra. For some, relying on the raw graph, as well as on the fly conversions and the maintenance of a 3D Pareto front might be more efficient. This model might also be more advantageous to \bestcop itself in some cases. This study is left for future works.
% Such investigations may also call forth the following question: is considering the number of segments of each path necessary?
% One may, for example, running Dijkstra based algorithms on the raw graph (relying on a PQ), and convert only the desired paths to segment lists
% afterward. Paths may turn out to exceed the MSD constraint, but could still be deployed relying on binding segments. This solution is however fairly risky. Binding segments should indeed be avoided, as they results in routing overhead and additional states to maintain in each routing node. Depending on the MSD constraint of the underlying hardware, and the nature of the network%(this requires specific analysis as it does neither return the 2COP nor the DCLC-SR solution)
% , this solution might lead to the use of too many binding segments.

% Overall, \bestcop is the only algorithm to provide safe guarantees regarding both its results and execution times when considering 2COP in all possible cases. By natively considering the number of segments, \bestcop ensures that the paths found are feasible without relying on the management of a 3D Pareto front, on the fly conversions, or binding segments, which could be very costly in worst cases. This is possible due to the fact that \bestcop deals more efficiently with dense networks than other state-of-the-art algorithms, as shown in this section, it does not rely on any PQ and perform efficient amortized Pareto front updates. Finally, \bestcop solves relevant TE-problems exactly in simple scenarios, or returns approximated solutions exhibiting strong, predictable and straightforward guarantees. Because of its ability to provide safeguards in all possible cases (regarding both its computation times and results), as well as its ability to deal with massive scale multi-area networks, \bestcop is an ideal candidate to be deployed for such TE flavors in IP networks.


==> clean_latex/sections/intro.tex <==
\section{Introduction}\label{sec:intro}

%cpe: parag on the needs of applications


%\textbf{Problem - delay.}
Latency is critical in modern networks for various applications. The constraints on the delay are indeed increasingly stringent.
For example, in financial networks, vast amounts
of money depend on the ability to receive information in real-time.
Likewise, technologies such as 5G slicing, in addition to requiring significant bandwidth availability,
demand strong end-to-end delay guarantees depending on
the service they aim to provide, e.g., less than 15ms for low latency applications such as motion control for industry 4.0, VR, or video games~\cite{5GSlicing}.
For such interactive applications, the latency is as critical as the \textit{IGP cost}.


%\textbf{Problem - delay + IGP cost.}
This Interior Gateway Protocol cost is defined as an additive metric that usually reflects both the
link's bandwidth and the operator's load
distribution choices on the topology.
Paths within an IGP are computed by minimizing this cost.
Thus, although delay constraints are increasingly important, they should not be enforced
to the detriment of the IGP cost.
With minimal IGP distances, the traffic benefits from high-bandwidth links and follows the
operator's intent in managing the network and its load.
With bounded delays, the traffic can benefit from paths allowing for sufficient
interactivity.
It is thus relevant to minimize the IGP cost while enforcing an upper constraint on the latency.
Computing such paths requires to solve DCLC, an NP-Hard problem standing for Delay Constrained Least Cost.\\
%(to allow the traffic to benefit from a high enough bandwidth and respect the operators' design),

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.3]{ersatz.pdf}
    \caption{Practical relevance of DCLC in the GEANT network. IGP costs are deduced from the bandwidth of each link. Depending on their needs (in terms of delay and bandwidth), applications can opt for three non-comparable paths between Frankfurt and Vienna.}
    \label{fig:DCLCGeant}
\end{figure}

%Fig description
\textbf{DCLC: a relevant issue.}
\red{Although one may expect the two metrics to be strongly correlated in practice, there are various cases where the delay and the IGP cost may be drastically different. For example, the IGP cost may have been tuned arbitrarily by the operator. Heterogeneous infrastructures between countries or geographical constraints may also create this effect. This can be illustrated on real networks, as displayed by
Fig.~\ref{fig:DCLCGeant}.}
This map is a sample of the GEANT transit network~\cite{GeantTopo}.
As fibers often follow major roads, we rely on real road distances to infer the propagation delay of each link while the bandwidth, and so the estimated IGP cost, matches the indications provided by GEANT. %cpe: add ref or footnote with the link to the information as it is public.
A green link has an IGP cost of 1 while the IGP cost is 2 and 10 respectively for the yellow and pink ones.

% When considering the couple Frankfurt-Vienna, this network exhibits three non-comparable (or \textit{non-dominated}) paths, forming the \textit{Pareto-front} of the paths between the two cities. These paths, as well as their delays and IGP distances, are provided in the legend.

\red{Note that the two metrics are not correlated, hence all three paths shown between Frankfurt and Vienna offer diverse interesting options. They are non-comparable (or \textit{non-dominated}) paths and form the \textit{Pareto-front} of the paths between the two cities.}
Either solely the delay matters and the direct link (in pink) should be preferred, or the ISP prefers to favor high capacity links, and the green path, minimizing the IGP cost, should be used.
The yellow path, however, offers an interesting compromise.
Out of all paths offering a latency well-below 10ms, it is the one minimizing the IGP cost. Thus,
it allows to provide strict Service-Level Agreement
($< 9$ms), while considering the IGP cost.
These kind of paths, retrieved by solving DCLC, provide more options by enabling tradeoffs between the two most important networking metrics. Applications such as videoconferences, for example, can then benefit both from real-time interactive voice exchange (delay) and high video quality (bandwidth).
In addition, IGP costs are also tuned to represent the operational costs. Any
deviation from the shortest IGP paths thus results in additional costs for the operator. For all these reasons, there exist a clear interest
for algorithms able to solve and deploy DCLC paths~\cite{SegmentR71:online}.
However and so far, while this problem has received a lot of attention in the last decades from the network research community~\cite{survey2018,survey2010}, no technologies were available for an efficient deployment of such paths.\\

%\textbf{Segment Routing.}
\red{\textbf{Segment Routing, MSD \& DCLC's (large-scale) rebirth.} Segment Routing (SR) is a vibrant technology gathering traction from router vendors,
network operators and academic communities \cite{I-D.matsushima-spring-srv6-deployment-status,ventre_segment_2020}.
% Example deployments include the facilitation of 5G deployments and inter data-center
% connectivity.
Relying on a combination of strict and loose source routing, SR enables to deviate the traffic from
the shortest IGP paths through a selected set of nodes and/or links by prepending routing instructions to the packet itself}.
Such deviations may for example allow to route traffic through a path with lower latency.
These deviations are encoded in the form of \textit{segments} within the packet itself. To prevent any packet forwarding degradation, the number of deviations \red{(\ie instructions)} one can encode is limited \red{to MSD (Maximum Segment Depth), whose exact value depends on the hardware}. While this technology is adequate to support
a variety of services, operators mainly deploy SR in the hopes of performing fine-grained and ECMP\footnote{Equal Cost Multi-Path}-friendly tactical Traffic-Engineering (TE)~\cite{SR4TE}, due to its reduced overhead compared to RSVP-TE \cite{filsfils2017segment}. Our discussion with network vendors further revealed a clear desire from operators to efficiently compute DCLC paths deployable with Segment Routing~\cite{SegmentR71:online}. Such a solution should thus not only
encompass Segment Routing, but also fare well on large-sized networks of several thousand of nodes, \red{as already observable in current SR deployments\cite{I-D.matsushima-spring-srv6-deployment-status}. Indeed, while we showed in~\cite{nca2020} that computing DCLC paths for Segment Routing (DCLC-SR) is possible in far less than a second on networks of up to $1000$ nodes, scaling to ten or a hundred times more routers remains an open issue.\\}


% We will discuss its overhead regarding DCLC, and its limitations in general: they are easy to mitigate in practice (as shown in Fig.\ref{fig:} illustrating that few deviations are enough for most usages).
%pointer to the required segments figure!
% cpe: cite the book on SR part 1 from Clarence and co. and cite some works that assume RSVP-TE for TE.

%\textbf{Goal.}
\textbf{Challenges.}
\red{In this paper, we extend our previous contribution, \bestcop (Best Exact Segment Track for the 2-Constrained Optimal Paths)~\cite{nca2020} to make DCLC-TE possible on (very) large scale networks.}
% reach computation times suitable for real-time routing.
\red{In order to achieve our goal, we solve several challenges: (i) efficiently cap, or even minimize, the number of segments
to consider the packet manipulation overhead supported by routers, (ii) scale with very large modern networks, and (iii) provide near-exact algorithms
with bounded error margin and strong guarantees despite the difficulty induced by considering
three metrics (cost, delay, and number of segments)\footnote{While difficult instances are unlikely to occur in practice, our algorithm can tackle even such corner cases. Thus, our proposal is not only efficient in practice but provably correct and efficient even for worst theoretical cases.}. We now briefly explain the main design aspects allowing us to solve these challenges. The latter will be explained more thoroughly in their dedicated sections.} \\


\textbf{Efficiently encompassing the Maximum Segment Depth constraint (MSD).}
\red{An SR router can only prepend up to \textit{MSD} routing instructions to a packet at line-rate, i.e., $\approx 10$ with the best current hardware.}
% Indeed, while SR can add instructions within the packets to guide them through the desired paths, the number of instructions is limited to \textit{MSD} ($\approx 10$ with good hardware).
\red{Although we find in our new study, shown in Section~\ref{ssec:nbseg} that this limit does not prevent from deploying most DCLC paths in practice (if not all in easy cases), this constraint must still be taken into account. If ignored, the computed paths have no guarantees to be deployable, as they may exceed MSD.}
%  when computing paths to ensure the completeness of the algorithm (\ie that the latter finds a feasible path if one exists.).

% Fortunately, \red{we find that} this constraint does not prevent SR from being used to deploy DCLC paths.
% According to our \red{new} study (Fig.~\ref{fig:nbseg}), the number of required segments does not exceed MSD for all constraints between 1 and 100ms in massive-scale transit networks ($\approx$ \num{50,000} nodes scattered in multiple areas) with realistic IGP costs.
% Nevertheless, the number of segments required to encode paths should still be taken into account.\red{If ignored, the paths computed by the algorithm may reveal themselves to require too many segments. To guarantee that our algorithm always returns deployable paths (if they exist), MSD should thus be taken into account nonetheless.}
%Indeed, in difficult cases, where computation times would increase significantly due to the difficulty of finding a suitable path for the constraints, the limit on MSD serves as a safeguard to cut the computation short. MSD prevents the rare use of inefficient paths with regard to the IGP cost.
\red{While this adds an additive metric to consider (the number of segments), \bestcop manages, through adequate data-structures and graph exploration, to natively manipulate the list of segments  
%instead of having to convert physical paths in segment lists and to control their size live, 
and ensure that paths requiring more than MSD segments are natively removed from the exploration space.}\\

%to be taken into account for computing the  paths,
%seemingly increasing the complexity of the traditional DCLC problem.
%By relying on a construct
%inherent to Segment Routing to guide the paths exploration, \bestcop natively considers the number
%of segments when computing constrained paths.

% Pas dit, mais s'il n'y a pas de zones, on peut toujours tenter de trouver des séparateurs
% cpe: fix the "et al."
\textbf{Towards massive-scale networks.}
\red{Our new proposal, \bestcope (\bestcop Extended), aims
at enabling fine-grained TE on massive-scale networks efficiently using a divide-and-conquer approach.}
Indeed, massive networks usually rely on a standard
physical and logical partitioning, as IGP protocols do not scale well as is.
By leveraging this decomposition and re-designing \bestcop to benefit from multi-threaded architectures, it becomes possible to solve DCLC-SR in a time suited for real-time routing.
To evaluate our contribution, we create a topology generator, YARGG, able to construct realistic massive-scale, multi-valuated, and multi-area topologies based on geographical data. In such cases, our extension solves DCLC-SR in $\approx$ 1 second for $\approx$ \num{100000} nodes.\\


\red{\textbf{Bounded error margin and practical concerns.}}
\red{DCLC is a well-known NP-Hard problem~\cite{536364}.
While there exist several ways to solve DCLC ~\cite{survey2018, survey2010}, they usually do not consider the underlying deployment technologies and real-life deployment constraints. We keep the latter at the core of our design. The nature of the concerned  TE paths allows us to consider a stable latency metric (the propagation delay). This is essential as
unstable metrics should not be considered nor advertised when performing routing~\cite{RFC7471,RFC8570}.
Furthermore, because of the arbitrary nature of the latency constraint and the inherent imprecision of
the delay measurement, we argue that an acceptable error margin regarding the delay constraint is acceptable
(more so than on the IGP cost). Our algorithm is designed to take advantage, if needed, of this acceptable
margin to returns the DCLC path efficiently in all situations to all destinations, with strong guarantees.\\}

% and often  do not offer any guarantees regarding either their computation time or optimality, both seemingly vital for a real-life deployment.


% However, it is worth noting that the delay constraints are usually formulated at the millisecond granularity and somewhat arbitrary.
% Besides, the real end-to-end experienced delay is often not measured. In practice, end-to-end latency is induced by the (variable) queueing delay and the (stable) propagation delay.


% Both delays may play an important part in the overall latency, though none can be stated to be the main factor~\cite{end2end}. When measuring delay for TE, it is strongly recommended to avoid measuring the queuing delay (through the use of a priority queue), so that the measurement remains stable~\cite{RFC7471,RFC8570}. Varying delay estimations may indeed lead to frequent re-computations, control-plane message exchanges and fluctuating traffic distribution.
% The propagation delay, deduced from
% the minimum observation within a large enough sampling
% window~\cite{perfmes}, is thus used as a stable lower-bound approximation of the end-to-end latency.
% Note that this is a pertinent estimation. In practice, \red{flows benefitting from DCLC paths will benefit from a queue with high priority and experience negligible queueing delays}.\red{In addition, the amount of traffic generated by such flows is pretty small. Consequently, not only is there no competition between DCLC flows and best-effort traffic, but DCLC flows are small enough to prevent competition between themselves. Thus, the experience delay is actually agnostic of the traffic load of the network, in our case.}
% Because of the arbitrary and imprecise nature of the constraints and the sole use of the propagation delay (whose measurement itself exhibits inherent limits in terms of trueness and accuracy), a bounded error margin is acceptable. \bestcop is designed to take advantage, if needed, of this acceptable margin.
% While \bestcop can return exact solutions, the latter can very easily be tuned
% to return approximated ones whose distances to the optimal solution can be bounded (within whatever desired acceptable error margin).\\

% cpe: we need to cite Jadin-near-optimal-infocom2019 here. (verifier si cette remarque est toujours pertinente)

\textbf{Summary and Contributions.}
By taking into consideration the operational deployment of constrained paths with SR, the current scale and structure of modern networks, as well as the practicality of the delay measures and constraints, \textbf{we designed BEST2COPE (BEST2COP Extended), a simple efficient algorithm able to solve DCLC-SR in $\approx$ 1s in large networks of $\approx$\num{100000} nodes}.


The main achievements of our proposal follow the organization of this paper:
\begin{itemize}
    \item In Section~\ref{sec:background}, we present SR in further details. \red{Compared to~\cite{nca2020}, we discuss the context and works related to DCLC in further detail. We also add an evaluation regarding the relevance of SR for deploying DCLC paths};
    \item In Section~\ref{sec:best2cop}, we formalize DCLC-SR and also its generalization (2COP). In particular, we describe the network characteristics we leverage and define the construct we use to encompass SR (in Sec.~\ref{sec:true} and Sec.~\ref{sec:sr-graph} respectively). \red{In Sec.~\ref{sec:flat}, we briefly summarize \bestcop (initially introduced in~\cite{nca2020} and detailed here in an appendix) and emphasize how it can easily benefit from multi-threaded architectures}.
\end{itemize}

\red{Besides the more detailed background and the evaluation of SR relevance, the main new contributions in this extension come in the last three sections:}

\begin{itemize}
    \item In Sec.~\ref{sec:areas}, we extend \bestcop to \bestcope, to deal with massive scale networks relying on area partitioning (as with OSPF with a single metric), making it able to solve DCLC efficiently in graphs of $\approx \num{100000}$ nodes;
    \item In Sec.~\ref{sec:complexity}, we formally define the guarantees brought by \bestcop and its versatility to solve several TE optimization problems at once (\ie the sub-problems of 2COP), as well as its polynomial complexity;
    \item Finally, in Section~\ref{sec:evaluation}, we
    present our large-scale topology generator, YARGG, and evaluate \bestcope on the resulting topologies and compare our proposal to the relevant state-of-the-art path computation algorithm.
\end{itemize}

% The rest of the paper is organized as follow:
% TODO%or use the itemize just before to do it...








%Segment Routing is being deployed on very large mobile networks~\cite{I-D.matsushima-spring-srv6-deployment-status}.


%New technologies, such as 5G slicing, require strong end-to-end guarantees, especially on the delay~\cite{5GSlicing}.


%Propagation delays are extracted from min/max/avg on various samples during a given window~\cite{RFC7810,perfmes}.


%The delay measurement should not vary significantly based upon the traffic load~\cite{RFC7810}.


% RFC 7810 While this document does not
%    specify how the performance information should be obtained, the
%    measurement of delay SHOULD NOT vary significantly based upon the
%    offered traffic load.  Thus, queuing delays SHOULD NOT be included in
%    the delay measurement.  For links such as Forwarding Adjacencies,
%    care must be taken that measurement of the associated delay avoids
%    significant queuing delay; that could be accomplished in a variety of
%    ways, including either by measuring with a traffic class that
%    experiences minimal queuing or by summing the measured link delays of
%    the components of the link's path.


% RFC 7810 In certain networks, such as, but not limited to, financial
%    information networks (e.g., stock market data providers), network-
%    performance information (e.g., latency) is becoming as critical to
%    data-path selection as other metrics.
%
%    In these networks, extremely large amounts of money rest on the
%    ability to access market data in "real time" and to predictably make
%    trades faster than the competition.  Because of this, using metrics
%    such as hop count or cost as routing metrics is becoming only
%    tangentially important.  Rather, it would be beneficial to be able to
%    make path-selection decisions based on performance data (such as
%    latency) in a cost-effective and scalable way.



% Additionally, the default measurement interval for all sub-TLVs
% SHOULD be 30 seconds.

% Announcements MUST also be able to be throttled using configurable
% inter-update throttle timers.  The minimum announcement periodicity
% is 1 announcement per second.  The default value SHOULD be set to 120
% seconds.

% Implementations SHOULD NOT permit the inter-update timer to be lower
% than the measurement interval.

% Furthermore, it is RECOMMENDED that any underlying performance-
% measurement mechanisms not include any significant buffer delay, any
% significant buffer-induced delay variation, or any significant loss
% due to buffer overflow or due to active queue management.


% \begin{itemize}
%     \item New technologies call for TE paths.
%     \item Legacy technologies, such as RSVP-TE, hindered the deployment of TE due to their lack of flexibility and scalability.
%     \item Segment Routing, a new TE technology, revived the possibility of deploying TE paths in large-scale networks.
%     \item Computing such paths leads to NP-Complete problems, whose complexity is even X by the technological constraint brought by SR.
%     \item Nevertheless, it has been shown that, by leveraging caracteristics inherent to operators networks and the aforementionned technological constraints, pratically relevant TE paths for SR can be computed in far less than a second in large networks of \num{1000} nodes~\cite{NCA2020}.
%     \item However, current modern network can be far larger and keep growing at a fast pace to keep up with new technologies and demands.
%     \item While computing TE paths can be done for fairly large networks, the
%     exponential and combinatorial natures of graphs seem to ultimately prohibit the usage of TE for networks of \num{10000} nodes or more~\cite{networksize}.
%     \item Such large networks usually rely on a logical and physical partitionning in area, mainly to allieviate the workload imposed on their IGP.
%     \item This partitionning can be leveraged for TE path computation as well. By computing TE-SR paths within each area before merging these results afterwards, deploying TE path on very large network becomes feasible.
%     \item We extend here our previous contribution, BEST2COP~\cite{NCA2020}, which computes TE paths (2COP, source to all dest...) for SR efficiently, to be able to deal with network of up to X nodes in less then X.
%     \item We evaluate BEST2COPE on topologies generated by a specifically designed topology generator, YARGG, which creates realistic multi-area topologies based on geographical locations, roads and designed recommended by network vendors. The generated topologies possess a realistic double valuation (IGP costs and delays).
%     \item We compare ...
% \end{itemize}


==> clean_latex/sections/problem.tex <==
\section{Problem Statement}\label{sec:problem}

\subsection{Basic Problem Formulation and Background}



%regarding here a constraint of 3 encapsulations at most).
% \QB{j'ai écrit plus clairement que Budapest est le segment utilisé (si j'ai bien compris), et j'ai enlever "regarding here a constraint of 3 encapsulations at most"}
%use again the fig of the intro to better illustrate and motivate..?



\paragraph{DCLC and True Measured Delays}
%In this section, we explain how and why
The characteristics of real ISP networks can be used to our advantage to solve DCLC.
First, althought NP-hard in theory, DCLC is pseudo-polynomial~\cite{gareycomputers} in practice.
As long as one of the two metrics is bounded, the exploration space is bounded as well.
More precisely, DCLC is polynomial in the smallest largest weight of
the two metrics $M_1$ and $M_2$ once translated to integers (\ie the numerical input)\footnote{Metric $M_0$ is omitted for now as this trivial distance is only required for SR and discussed in details later. While dealing with a three-dimensional Pareto front seems more complex at first glance, we will show that SR eventually reduces the exploration space because its operational constraint is very tight in practice and easy to handle efficiently.}.
Consequently, as long as one of these two metrics possesses only a limited number of distinct values, DCLC is tractable and can be solved efficiently as the Pareto front of the paths' distances is bounded in size.

% The delay is nice
This bounded metric can possess a coarse accuracy by nature, and/or its associated constraint can be small enough to sufficiently reduce the number of values within the solution space.
Although our solution can be adapted to fit any metric, we argue that $M_1$, the propagation delay, will, by design and most of the time, have less distinct values than $M_2$ in the general case.
% Why is the delay nice ?
First, for constrained TE paths, the delay constraint is likely to be very strict (10ms or less). Second, while the delay of a path is generally represented by a precise number in memory (at the nano-second grain or even less), the actual accuracy, i.e the trueness, of the measured delay is coarser (at the micro-second unit at best).
%ISPs are aware that measured delays are an estimation, not a guarantee.
Propagation delays (usually measured with softwares like OWAMP~\cite{RFC4656}/TWAMP~\cite{RFC5357}) have limited accuracy, even with efficient hardware PTP time-stamping systems or accurate two-way delay link estimators. Due to both its inherent variation depending on physical properties, clock synchronization, or inconstant packet processing delays~\cite{RFC7679, RFC2681}, we argue that truly distinguishing the delay of a path at the granularity of the micro-second is very challenging.
%if not impossible nowadays in most ISPs.

Floating numbers representing the delays can be truncated to integers, e.g. taking 0.1ms as unit to achieve a reasonable tradeoff regarding typical constraints between 1 and 10ms.
This allows to easily bound the number of possible non-dominated distances to $c_1 \times t$, with $t$ being the supported level of accuracy of $M_1$ (the inverse of the unit of the delay grain, here 0.1ms). %, and $c_1$ the delay constraint.
For example, with $c_1 = 100$ms and a delay grain of 0.1ms ($t = \frac{1}{0.1} = 10$), we have only $1000$ distinct (truncated) non-dominated pairs of distances to track at worst.
For each truncated delay, it becomes then sufficient to store only the best $M_2$-distance indexed on its respective $M_1$-distance, leading to a predictable, reduced Pareto front that can be stored and managed in
a static array. In the remaining of the paper, $\Gamma$ denotes the size allocated in memory for this Pareto front array. When the actual trueness, i.e the real level of accuracy is lower (or equal) than the $t$ we rely on, we consider the stored delay to be exact, \ie discretized but with no loss of relevant information.
Otherwise, the correctness is no longer granted because one can opt for performance rather than increasing $\Gamma$ (to remain exact at the detriment of the efficiency); with such an option, our algorithm is nevertheless able to provide predictable guarantees, i.e. a bounded error margin on the delay constraint, discussed in details in section \ref{sec:b2coplimits}.



==> clean_latex/sections/related.tex <==
\section{Related Work}


QoS routing and TE being popular subject for several years, it is impossible to showcase here all past work. However, there are several extensive surveys ~\cite{survey02,survey2018,survey2010} that exhibit most of the solutions developed in the past decades.

Specific to DCLC,
DCUR~\cite{dcur} explores the network by extending paths either
through the least-delay or the least-cost path.
DCUR has been combined with Bellman Ford to create DCBF~\cite{dcbf}, which guesses promising paths
through an estimated cost.
Closer to our work, Constrained Bellman-Ford~\cite{CBF94}, solves
DCLC exactly by exploring paths in a greedy fashion through a priority
queue indexed on their delay. CBF was extended in ~\cite{EBFA01}, which adds two heuristics to 
ease the problem, first by discretizing all metrics but one, second by only extending the best $k$ paths.


Our work comes with several
advantages, simplicity being its main strength.
We propose an all-in-one solution, that solves 2COP and returns the corresponding list of segments.
Our approach is an exact algorithm with a straight-forward bounded
worst-case time complexity, with no parameters
requiring tuning. While other works solving DCLC usually detach
path computations and their deployment, we are, to the best of our knowledge,
the first ones to propose an algorithm that leverages and takes into account SR deployment constraints to solve DCLC for SR.
% Our data-structure can be adapted to fit realistic and worst-case scenario.
In addition, while not all works evaluate the time complexity of their solution, or do so on limited topologies, we provide extensive evaluations on random and real large topologies, which bound
the worst-case time complexity of \bestcop for the 2COP problem.



==> sections/bio.tex <==
% !TEX root = ./paper.tex
\vspace{-1cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {JRL.pdf}}]{Jean-Romain Luttringer} received his master's degree in
  Computer Science from the University of Strasbourg (France) in 2019, where
  he is currently a Ph.D. candidate within
  the Networks Research Group of the ICube laboratory. His research interests
  includes routing and path computation.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {alfroy.jpeg}}]{Thomas Alfroy} received his master's degree in Computer Science from the University of Strasbourg (France) in 2021. He is currently a Ph.D student within the Network Research Group of the ICube laboratory. His research topics are Network anomaly detection and BGP.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {Quentin.pdf}}]{Quentin Bramas}  received a M.Sc. in Computer Science from
  Nancy University (France, 1972), a Ph.D. in Computer Science from Cornell
  University (USA, 1976).
  % and a ``Doctorat d'Etat'' from the University of Strasbourg (France, 1983).
  He joined the Department of Computer Science from the same University where he was successively appointed as Assistant Professor, Associate Professor, and Full Professor (1984). He led the Network and Protocol group of the LSIIT Laboratory and is now retired. His research interests included
  % routing, multicasting,
  traffic engineering and Internet cartography.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {Pascal.pdf}}]{Pascal M\'erindol} received his Ph.D. degree from the
  University of Strasbourg (France) in 2008. Then, he spent two years in Belgium
  at the Universit\'e catholique de Louvain as a post-doctoral researcher. He is now
  Associate Professor at the Networks Research Group of the ICube laboratory in the University of Strasbourg. His main research topics are routing and Internet measurements.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
  [{\includegraphics[width=0.9in,height=1.125in,clip,keepaspectratio]
  {Cristel.JPG}}]{Cristel Pelsser} received the Ph.D. degree from the Université catholique de Louvain (UCLouvain), Belgium. She has spent nine years working for ISPs. She has been a Professor with the University of Strasbourg since November 2015. She leads a team of researchers focusing on core Internet technologies. Her aim is to facilitate network operations, and to avoid network disruptions.
\end{IEEEbiography}


==> sections/problem.tex <==
\section{Problem Statement}\label{sec:problem}

\subsection{Basic Problem Formulation and Background}



%regarding here a constraint of 3 encapsulations at most).
% \QB{j'ai écrit plus clairement que Budapest est le segment utilisé (si j'ai bien compris), et j'ai enlever "regarding here a constraint of 3 encapsulations at most"}
%use again the fig of the intro to better illustrate and motivate..?



\paragraph{DCLC and True Measured Delays}
%In this section, we explain how and why
The characteristics of real ISP networks can be used to our advantage to solve DCLC.
First, althought NP-hard in theory, DCLC is pseudo-polynomial~\cite{gareycomputers} in practice.
As long as one of the two metrics is bounded, the exploration space is bounded as well.
More precisely, DCLC is polynomial in the smallest largest weight of
the two metrics $M_1$ and $M_2$ once translated to integers (\ie the numerical input)\footnote{Metric $M_0$ is omitted for now as this trivial distance is only required for SR and discussed in details later. While dealing with a three-dimensional Pareto front seems more complex at first glance, we will show that SR eventually reduces the exploration space because its operational constraint is very tight in practice and easy to handle efficiently.}.
Consequently, as long as one of these two metrics possesses only a limited number of distinct values, DCLC is tractable and can be solved efficiently as the Pareto front of the paths' distances is bounded in size.

% The delay is nice
This bounded metric can possess a coarse accuracy by nature, and/or its associated constraint can be small enough to sufficiently reduce the number of values within the solution space.
Although our solution can be adapted to fit any metric, we argue that $M_1$, the propagation delay, will, by design and most of the time, have less distinct values than $M_2$ in the general case.
% Why is the delay nice ?
First, for constrained TE paths, the delay constraint is likely to be very strict (10ms or less). Second, while the delay of a path is generally represented by a precise number in memory (at the nano-second grain or even less), the actual accuracy, i.e the trueness, of the measured delay is coarser (at the micro-second unit at best).
%ISPs are aware that measured delays are an estimation, not a guarantee.
Propagation delays (usually measured with softwares like OWAMP~\cite{RFC4656}/TWAMP~\cite{RFC5357}) have limited accuracy, even with efficient hardware PTP time-stamping systems or accurate two-way delay link estimators. Due to both its inherent variation depending on physical properties, clock synchronization, or inconstant packet processing delays~\cite{RFC7679, RFC2681}, we argue that truly distinguishing the delay of a path at the granularity of the micro-second is very challenging.
%if not impossible nowadays in most ISPs.

Floating numbers representing the delays can be truncated to integers, e.g. taking 0.1ms as unit to achieve a reasonable tradeoff regarding typical constraints between 1 and 10ms.
This allows to easily bound the number of possible non-dominated distances to $c_1 \times t$, with $t$ being the supported level of accuracy of $M_1$ (the inverse of the unit of the delay grain, here 0.1ms). %, and $c_1$ the delay constraint.
For example, with $c_1 = 100$ms and a delay grain of 0.1ms ($t = \frac{1}{0.1} = 10$), we have only $1000$ distinct (truncated) non-dominated pairs of distances to track at worst.
For each truncated delay, it becomes then sufficient to store only the best $M_2$-distance indexed on its respective $M_1$-distance, leading to a predictable, reduced Pareto front that can be stored and managed in
a static array. In the remaining of the paper, $\Gamma$ denotes the size allocated in memory for this Pareto front array. When the actual trueness, i.e the real level of accuracy is lower (or equal) than the $t$ we rely on, we consider the stored delay to be exact, \ie discretized but with no loss of relevant information.
Otherwise, the correctness is no longer granted because one can opt for performance rather than increasing $\Gamma$ (to remain exact at the detriment of the efficiency); with such an option, our algorithm is nevertheless able to provide predictable guarantees, i.e. a bounded error margin on the delay constraint, discussed in details in section \ref{sec:b2coplimits}.



==> sections/related.tex <==
\section{Related Work}


QoS routing and TE being popular subject for several years, it is impossible to showcase here all past work. However, there are several extensive surveys ~\cite{survey02,survey2018,survey2010} that exhibit most of the solutions developed in the past decades.

Specific to DCLC,
DCUR~\cite{dcur} explores the network by extending paths either
through the least-delay or the least-cost path.
DCUR has been combined with Bellman Ford to create DCBF~\cite{dcbf}, which guesses promising paths
through an estimated cost.
Closer to our work, Constrained Bellman-Ford~\cite{CBF94}, solves
DCLC exactly by exploring paths in a greedy fashion through a priority
queue indexed on their delay. CBF was extended in ~\cite{EBFA01}, which adds two heuristics to 
ease the problem, first by discretizing all metrics but one, second by only extending the best $k$ paths.


Our work comes with several
advantages, simplicity being its main strength.
We propose an all-in-one solution, that solves 2COP and returns the corresponding list of segments.
Our approach is an exact algorithm with a straight-forward bounded
worst-case time complexity, with no parameters
requiring tuning. While other works solving DCLC usually detach
path computations and their deployment, we are, to the best of our knowledge,
the first ones to propose an algorithm that leverages and takes into account SR deployment constraints to solve DCLC for SR.
% Our data-structure can be adapted to fit realistic and worst-case scenario.
In addition, while not all works evaluate the time complexity of their solution, or do so on limited topologies, we provide extensive evaluations on random and real large topologies, which bound
the worst-case time complexity of \bestcop for the 2COP problem.


